DRust: Language-Guided Distributed Shared Memory with Fine Granularity, Full Transparency, and Ultra Efficiency

Despite being a powerful concept, distributed shared memory (DSM) has not been made practical due to the extensive synchronization needed between servers to implement memory coherence. This paper shows a practical DSM implementation based on the insight that the ownership model embedded in programming languages such as Rust automatically constrains the order of read and write, providing opportunities for significantly simplifying the coherence implementation if the ownership semantics can be exposed to and leveraged by the runtime. This paper discusses the design and implementation of DistR, a Rust-based DSM system that outperforms the two state-of-the-art DSM systems GAM and Grappa by up to 2.64x and 29.16x in throughput, and scales much better with the number of servers.

==> QA.tex <==
% \section{Q\&A}

% \begin{itemize}
%     \item Q1. I was thinking local vs. remoteable. What kinds of benefits do you provide by having 3 categories: remoteable(regular), mustremote, and mustlocal?
%     \begin{itemize}
%         \item A. It is more like a 2-step thing. First, by having mustlocal and mustremote, we give the programmers the right to control the place of each object. Then programmers can write code to achieve great application performance because they know better what their system is doing. But annotating each object is a way too big burden for programmers. So I add this remoteable type. Every object without annotation is remoteable by default. It means it is managed by underlying swap system. Programmers can be freed from managing data that are not performance sensitive.
%     \end{itemize}
%     \item Q2. What would be the runtime semantics of type conversion operators? What kinds of type conversion do you?
%     \begin{itemize}
%         \item A. All three types(with the same object class) can be converted between one another. Its meaning is straightforward, just to move the object. For example, when we convert a remote type to local type through $a=b$ where $a$ is local and $b$ is remote, it means we fetch that content in object $b$ into local server and write it to $a$. 
%     \end{itemize}
%     \item Q3. What are the violations that you can detect statically that is not too restrictive version of “local must be local” and “remote must be remote”.
%     \begin{itemize}
%         \item A. I want to check and guarantee that regular functions only access data with local and regular types, and remote functions only access data with remote types. Any violation should be detected during compilation time.
%     \end{itemize}
%     \item Q4. If we go with the Rust style ownership type, we are essentially having only one reference that could have a write privilege? What do we then lose in terms of “data structure” that can be expressed and optimized in memory disaggregation setting?
%     \begin{itemize}
%         \item A. It is sometimes hard to implement some data structures like "doubly linked list".
%     \end{itemize}
%     \item Q5. How are we distinguishing computation as local vs remote when the types are in 3 different types? Are we also going to add type annotation (or suffixes) where the computation is designated to be must local, must remote, or could be both?
%     \begin{itemize}
%         \item A. Yes, we need to annotate functions to be local or remote. Functions annotated with "remote" are executed on the remote memory server, while functions without any annotations (regular functions) are executed on the local server. 
%     \end{itemize}
%     \item Q6. If there are multiple remote servers, how do you check the legality of computation? For example remote server 1 and remote server 2. 
%     \begin{itemize}
%         \item A. We currently do not consider this scenario in our setting.
%     \end{itemize}
% \end{itemize}

==> deprecated/design.tex <==
\section{Design}
Hardware Setting: CPU Server + Memory Server
\begin{itemize}
    \item Programmers should be aware of the fact that resource is disaggregated and know the total amount of resource (how much is local, how much is remote).
    \item The type system should guarantee that every access in local function is to local data, every access in remote function is to remote data.
\end{itemize}

    
\subsection{Type Annotations \label{sec:annotation}}
\begin{itemize}
    \item Regular variable: For variables without annotation, it means that they store an object that could be remote or local.  And this kind of data could be swapped in and swapped out through swap systems.
    \item Local variable: For variables with annotation $l$, it means that they store an object that must be local on the CPU server
    \item Remote variable: For variables with annotation $r$, it means that they store an object that resides only on remote memory server
\end{itemize}

\begin{lstlisting}[language=Rust, style=boxed]
// Struct A stored in local stack
a1: A@l;  
// Struct A stored in remote stack
a2: A@r;  
// Struct A stored in stack, and could be swapped in and out
a3: A;    
\end{lstlisting}


There are two operations when assigning values: Move and Copy. For both of them, we can directly move/copy values between the same type with different place annotations.


\subsection{Struct Definition}

Inside the struct, we can also declare boxed references with a special annotations @t. For boxed references without annotation, it means that they point to an object that could be remote or local. For boxed references with annotation $t$, it means that they point to an object that must be together with the current object. For boxed references with annotation $l$ or $r$, then it is the same as Section~\ref{sec:annotation}.

For non-box fields, we do not need to annotate them because they are inside the struct so they are in the same place. And for references to stack objects, we cannot annotate it with @t because when we automatically move it with its outside struct, we need to put it onto stack but we cannot find a place to put it.

\begin{lstlisting}[language=Rust, style=boxed]
struct A {
	b1: Box<B@t>,
	b2: B,
	b3: &B
}

let a: A@l = ...;
// b1 is of type Box@l<B>
\end{lstlisting}


\subsection{Object Creation}

We have two functions to create a box value.

\begin{itemize}
    \item \textbf{new} is the default keyword to use to create an object. It will allocate an object on the local heap.
\item \textbf{rnew} directly allocates an object on the remote heap.
\end{itemize}

\begin{lstlisting}[language=Rust, style=boxed]
let mut a1: A@l = A@l{field1: 0, field2: 0}
let mut a2: Box@l<A@l> = Box::new(A{field1: 0, field2: 0})


let mut a1: A@r = A@r{field1: 0, field2: 0}
let mut a2: Box@l<A@r> = Box::rnew(A{field1: 0, field2: 0})

\end{lstlisting}

\subsection{Function Execution}
\begin{itemize}
    \item Regular functions can only access local variables and regular variables. 
    \item Remote functions can only dereference and access remote variables. It has suffix: \_\_REMOTE
\end{itemize}


\subsection{Static Fields}

Rust does not support static fields in struct so we do not need to consider that here.

\subsection{CPU/Memory Server Sync}

Our type system guarantees that no data would be accessed by the CPU server and memory server at the same time. 


\subsection{Example: Single Linked List}

\subsubsection{Single Machine Version}
\begin{lstlisting}[language=Rust, style=boxed]
struct BigVal {
    nums: [i32; 1024]
}

struct Node {
    key: i32,
    val: Box<BigVal>,
    next: Option<Box<Node>>
}

struct LinkedList {
    length: u32,
    head: Option<Box<Node>>
}

fn insert_at_head(mut l: LinkedList, obj: i32) -> LinkedList{
    let mut node = Box::new( Node {key: obj, val: Box::new(BigVal {nums: [obj; 1024]}), next: None});
    node.next = l.head;
    l.head = Some(node);
    l.length += 1;
    l
}

fn get_sum_by_key(l: &LinkedList, key: i32) -> i32 {
    iterate_node(&l.head, key)
}

fn get_sum(bigval: &BigVal) -> i32 {
    let mut s = 0;
    for n in 0..1024 {
        s += bigval.nums[n];
    }
    s
}

fn iterate_node(node: &Option<Box<Node>>, key: i32) -> i32 {
    match node {
        None => 0,
        Some(node) => {
            if key == node.key {
                get_sum(&(*(node.val)))
            } else {
                iterate_node(&node.next, key)
            }
        }
    }
}

// test
fn main() {
    let mut list = LinkedList{length: 0, head: None};
    for n in 0..1024 {
        list = insert_at_head(list, n);
    }
    
    for n in 23..30 {
        println!("key is {}, sum is {}", n, get_sum_by_key(&list, n));
    }
}
\end{lstlisting}


\subsubsection{Disaggregated Version}
\begin{lstlisting}[language=Rust, style=boxed]
struct BigVal {
    nums: [i32; 1024]
}

struct Node {
    key: i32,
    val: Box<BigVal@r>,  // It means that val points to an remote BigVal Object
    next: Option<Box<Node@t>>
}

struct LinkedList {
    length: u32,
    head: Option<Box<Node@t>>
}

fn insert_at_head(mut l: LinkedList@l, obj: i32) -> LinkedList{
    let mut node: Box<Node@l>>  = Box::new( Node {key: obj, val: Box::rnew(BigVal {nums: [obj; 1024]}), next: None}); // Remote create object
    node.next = l.head;
    l.head = Some(node);
    l.length += 1;
    l
}

fn get_sum_by_key(l: &LinkedList@l, key: i32) -> i32 {
    iterate_node(&l.head, key)
}

fn get_sum__REMOTE(bigval: &@r(BigVal@r)) -> i32 {
    let mut s = 0;
    for n in 0..1024 {
        s += bigval.nums[n];
    }
    s
}

fn iterate_node(node: &Option<Box<Node@l>>, key: i32) -> i32 {
    match node {
        None => 0,
        Some(node) => {
            if key == node.key {
                get_sum__REMOTE(&(*(node.val)))
            } else {
                iterate_node(&node.next, key)
            }
        }
    }
}

// test
fn main() {
    let mut list: LinkedList@l = LinkedList{length: 0, head: None};
    for n in 0..1024 {
        list = insert_at_head(list, n);
    }
    
    for n in 23..30 {
        println!("key is {}, sum is {}", n, get_sum_by_key(&list, n));
    }
}
\end{lstlisting}



















































% \subsection{Class Definition}

% Inside the class, we can also declare variables.

% \begin{itemize}
%     \item For references without annotation, it means that they point to an object that could be remote or local
% \item For references with annotation $t$, it means that they point to an object that must be together with the current object.

% \end{itemize}

% \begin{lstlisting}[language=Java]
% public class A {
% 	B@t b1;
% 	B b2;
% }

% A@l a;
% //a.b1 is on the same server

% a.b1 = b2
% \end{lstlisting}


% \subsection{Object Creation}

% We have two keywords to create an object.

% \begin{itemize}
%     \item \textbf{new} is the default keyword to use to create an object. It will allocate an object on the local memory.
% \item \textbf{rnew} directly allocates an object on the remote memory where the reference resides.
% \end{itemize}

% \begin{lstlisting}[language=Java]
% A@l a1 = new A();
% A a2 = new A();
% A@r a3 = rnew A();
% \end{lstlisting}

% \subsection{Function Execution}

% The functions inside a class are all executed on the server where the object resides. 

% \begin{lstlisting}[language=Java]
% public class A {
% 	int result;
% 	B@t b1;

% 	// parameter b1 must reference a local object on the same server
% 	void add(B@t b2) {
% 		B@l b1_prime = b1;
% 		int value1 = b1_prime.get_value();
% 		B@l b2_prime = b2;
% 		int value2 = b2_prime.get_value();
% 		result = value1 + value2;	
% 	}

% 	void add(B@t b2) {
% 		B@r b1_prime = remote(b1);
% 		**int value1 =** fetch(**b1_prime.get_value()); // Type inferences**
% 		B@r b2_prime = remote(b2);
% 		int value2 = fetch(b2_prime.get_value());
% 		result = value1 + value2;	
% 	}
% }

% // object for A, should be in the same place as b1, and b2 to be added is also in the same place. 
% // scenario 1. 
% A@l a = new A(); 
% B b = new B(); // local object B is a super type B@l
% a.b1 = b // legal because b is a local object. 

% // scenario 2 
% A@l a = new A(); 
% B b = rnew B(); // remote object B is a super type B@l
% a.b1 = b // illegal 
% a.b1 = local(b); // legal 
 
% // scenario 3
% A@r a = rnew A(); //remote  
% B b = rnew B(); // remote object B is a super type B@l
% a.b1 = local(b); // legal the target location is left hand side of expression 
% a.b1 = b //illegal because remote location of b could be different from a remote location of a.b1

% // scenario 4
% A@r a = rnew A(); //remote  
% B b = new B(); // local object b of B@r can be assigned type B  
% a.b1 = local(b) // explicitly tell a target location to migrate
% //I want to put a local b to remote a. swapout happens. 

% A@r a = rnew A();
% B@l b = new B();
% a.add((b, a));
% \end{lstlisting}

% ---

% This design works for single-thread simple programs without static variables. We need to deal with static fields and multi-threads.

% \subsection{Static Fields}

% Objects that spread across different can share the same static variable. But we can solve this problem by adding a class object.

% \begin{itemize}
%     \item Static variables cannot be annotated with $t$
%     \item Getting and changing value of static variables should be done through function calls. We can implement it as if we have an object of that class. It possesses the static fields.
% \end{itemize}


% An example is shown below

% \begin{lstlisting}[language=Java]

% public class A {
% 	static int result;

% 	// The following code can be generated automatically
% 	A static_obj;
% 	void set_result_static(int 0) {
% 			static_obj.set_result(0);
% 	}
% 	int get_result_static() {
% 			static_obj.get_result();
% 	}
% }

% A@l a;
% a.set_result_static(0);
% int b = a.get_result_static();

% \end{lstlisting}

% \subsection{Multi-References}

% \subsection{Multi-Threads}

% This might be the biggest challenge in our design. We cannot guarantee correctness for multi-threading program. Objects can be read/written on different servers. Example shown below:

% \begin{lstlisting}[language=Java]

% public class A {
% 	int result;
% }
% public class B {
% 	A a;
% }

% // Thread 1 on Server 1
% void func1(B b) {
% 	A@l a = new A();
% 	a.result = 0;
% 	B@l b_local = local(b);
% 	b.a = a;  // Step 1

% 	int c = a.result;  // error! Because it still assumes a is on server 1. 
% 										 // Either c is wrong or there can be some segmentation fault.
% }

% // Thread 2 on Server 2:
% void func1(B b) {
% 	B@l b_local = local(b);
% 	A@l a = local(b_local.a);
% 	a.result = 100; // Step 2, a now is on Server 2.
% }
% \end{lstlisting}

% \subsection{design choices}

% \subsubsection{Correctness Ensured by Programmers}

% ~~We let programmers take care of multithread issues. They can deal with this with careful synchronization and data partition mechanism.~~ 

% \subsubsection{Correctness Ensured by Languages}

% Ownership of objects belongs to threads. We let thread own the object that it has local references to. If the other thread wants to migrate an object. It needs to first check if that object is being owned by other threads. If not, then this operation is invalid. If so, the migration function migrates the object to that server and let the other thread own the object.

% If the current thread is not going to use an object again. Then it should give up the ownership of the object.


% \begin{lstlisting}[language=Java]
% public class A {
% 	int result;
% }
% public class B {
% 	A a;
% }


% // Case 2:
% // Thread 1 on Server 1
% void func1(B b) {
% 	A@l a = new A();
% 	a.result = 0;
% 	B@l b_local = local(b);
% 	b.a = a;  // Step 1
% 	int c = a.result;  
% 	release(a);
% }

% // Thread 2 on Server 2:
% void func1(B b) {
% 	B@l b_local = local(b);
% 	A@l a = local(b_local.a); // wait until b_local.a is released.
% 	a.result = 100; 
% }

% // Implementation of release
% void release(A@t a) {
% 	A ar = a;
% 	change_ownership(a, NULL);
% 	a = NULL;
% }
% \end{lstlisting}

==> deprecated/intro_dep.tex <==

Distributed Shared Memory (DSM) offers the illusion of a single, contiguous memory space that can be accessed by multiple processors or machines.

Distributed Shared Memory (DSM) serves as a critical abstraction layer that facilitates the sharing of memory resources across multiple nodes in a distributed computing environment, effectively bridging the gap between local and remote memory access. Although DSM was a popular concept in the formative years of distributed computing, its widespread adoption was hindered due to performance bottlenecks caused by low network speeds. However, the advent of new, high-speed networking technologies has reinvigorated the field, making DSM an increasingly viable and attractive option for enabling efficient data sharing and communication among distributed systems.

The field of distributed computing has undergone a remarkable evolution to cope with the challenges posed by the data explosion and the escalating complexity of modern computing tasks. By integrating several interconnected computers or nodes, distributed systems facilitate parallel task execution, leading to enhanced performance, scalability, and reliability. 
Two primary programming models have emerged in this field: the shared-nothing model and the shared-memory model. In the shared-nothing model, each node in the system operates independently with its private memory and storage, requiring explicit communication for data sharing between nodes. However, this model often requires manual data partitioning and significantly increases programming complexity.
In contrast, the distributed shared memory (DSM) model provides a programming paradigm that significantly mitigates the complexity associated with developing distributed applications. Unlike the shared-nothing model, DSM presents a unified memory space across multiple nodes, providing a programming paradigm similar to developing multi-threaded applications on a single machine. However, maintaining memory consistency in DSM systems has been a formidable challenge, primarily due to network speed limitations, which create a significant performance bottleneck and thwart the realization of DSM's full potential. This problem caused a decrease in its popularity after the 1990s.
% Memory consistency is crucial because it ensures all nodes have the same view of the shared memory, which is essential for the correct execution of distributed applications.

Recent advancements in network technology offer new opportunities for enhancing DSM system performance. Several new DSM systems designed to leverage these faster networks have been proposed. One primary strategy employs a write-through-like approach, routing each read/write operation directly to the data resident node via a high-speed network, as exemplified by~\cite{sdsm-atc15}. However, this approach neglects data locality considerations, potentially resulting in inefficient data access patterns. Despite the bandwidth of current fast networks like Remote Direct Memory Access (RDMA) approaching that of local memory access, their latency remains orders of magnitude longer than local memory. \shi{The shortcoming does not feel very clear. Maybe we can put the latency constraint in the front and say that this approach eliminates the possibility of \textit{caching} remote data, which can be critical to the performance. The reader may not immediately realize what "data locality" means in this setting. Also 2 minor points: 1. "write-through-like" only characterizes the behavior of writing, maybe change a word, or just say every remote access is fulfilled directly by the home node of the data via the network. 2. "resulting in inefficient data access patterns" feels ambiguous. The design does not introduce access patterns with bad performance. It is because that data cannot be cached that makes the system inefficient for applications that can benefit from caching (which are most applications).}

An alternative strategy implements a directory-based \shi{cache} protocol, assigning a 'home node' to each small data block. This home node maintains the states and locations of cache copies, as exemplified by~\cite{cai2018efficient,wang2021concordia}. Although this method considers data locality and shows improved performance on a set of applications than the first method, it still incurs a high synchronization overhead due to the requirement for several round trips of network access to do every cache invalidation operation, preventing satisfactory performance. \shi{Maybe we can say round trips are required for all kinds of synchronization operations (or change of cache states), not only invalidations. (e.g., Exclusive -> Shared.)} As demonstrated in section~\ref{sec:motvation}, the open-sourced state-of-the-art GAM~\cite{cai2018efficient} exhibits a \mhr{Y$\times$} slowdown for a simple multi-threaded text-processing application compared with running on a single machine with sufficient resources.

% and result in wasted resources. For instance, in a typical piped multi-threaded program, where threads run on different physical nodes executing distinct tasks, a set of synchronization operations may be unnecessary if a thread won't access a certain data block again in the near future. However, the underlying memory management system doesn't know this semantic information of applications, so it performs frequent synchronization to maintain memory consistency. We argue that if such information can be transferred from applications to memory management systems, performance can be significantly improved. \shan{Leveraging semantic information for enhanced performance should be our core contribution and main insights. However, bringing up this while telling GAM, may narrow our scope down, into solving a sub-problem introduced by the GAM method. Maybe we should highlight our problem scope when explaining our core insights and contribution.}

We observed that many synchronizations required to maintain memory consistency are superfluous and hence wasted if we could leverage the semantic information from the applications. \shan{Maybe including the figure and detailed explanation in the motivation part. In that case, we can have the space to explain the setting more clear.. Placing it in the introduction may require a detailed explanation which may distract from the core storyline.} For example, figure A(a) shows a typical piped multi-threaded program, where threads run on different physical nodes executing distinct tasks. Thread 1 cached and processed the data block A whose home node is node 0 and passed its reference to thread 2. Thread 2 would read and write data block A. But before reading and writing the data, there is a set of synchronization operations (\textcircled{2}-\textcircled{4}, \textcircled{5}-\textcircled{8}) that need to be done to maintain memory consistency. 
These operations are unnecessary in this scenario because thread 1 will not access this data block again. With this semantic information, the optimal method is that thread 2 directly reads data from node 1 and does no synchronization operations, which causes much less communication cost. However, the underlying memory management system does not know this semantic information of applications, so it has to performs frequent synchronization to maintain memory consistency. We argue that if such information can be transferred from applications to memory management systems, performance can be significantly improved. \shi{I also feel this paragraph may be too detailed for the introduction and may be offloaded to the motivation.} \shan{Should we compare both Grappa-like methods and GAM-like methods with ownership? In that case, we can motivate that DRust, with semantic information, is a more efficient solution than current state-of-the-art memory consistency maintaining methods in DSM, which enlarges our problem scope.}

\begin{figure*}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[scale=.8]{figs/intro-exp-a.pdf} & 
     \includegraphics[scale=.8]{figs/intro-exp-b.pdf}\\
     (a) Directory-based Protocol & (b) DRust's Ownership Transfer 
     \end{tabular}
    \caption{Semantic information helps reduce synchronization overhead. \label{fig:intro-example}}
\end{figure*}

In this context, the ownership model becomes significant relevant. This model, which has been studied in the programming language community for decades, is the basis of the new Rust programming language, which has proven its success by being adopted in many industry applications. Rust's ownership model offers several advantages, including memory safety, no garbage collector, no manual memory management, no data races, and superior performance. Upon inspection, it becomes clear that Rust's ownership model's benefits extend beyond single-machine settings. Indeed, we argue that it can provide a perfect bridge for transferring semantic information between applications and the memory management system.
The key rule in Rust's ownership model is that each value has a unique variable as its owner at any time. It allows references to values but enforces the rule that at any given time, either one mutable reference or any number of immutable references can exist to the same data, but never both. This is the exact information that the underlying memory management system needs. For instance, the exclusive dirty state for each data block corresponds to Rust's unique owner or mutable reference concept; the shared state aligns with the concept of immutable reference borrowing. \shi{This analogy between ownership concepts and cache line states feels abrupt. After saying "this is what the underlying memory management system needs." we should give further explanation on this point, like how this concept passes semantic information to the memory management system.} \shan{Maybe we shouldn't include the analogies in the introduction, since the mappings between underlying system support and Rust ownership are very hard for me to follow (Need to think A. What role do \textit{the exclusive dirty state,  the shared state} play in memory management system for DSM, how do they affect the performance? B. What are the definitions of the Rust ownership concepts? C. Why and how do they map together?) Besides, the mappings also narrow down our scope, since they are only for the directory-based protocol, and the comparison between write-through-like methods with Rust ownership is not mentioned. Maybe we can switch to another angle: which kinds of semantic information can be utilized to ease the underlying memory management system as well as improve performance, which is provided naturally from ownership. Then explain how ownership provides the semantic information.} \shan{How / In which cases does DRust achieve better performance than the grappa model is not very clear. How do we use the semantic information for better performance? (Read cache for immutable reference borrowing, .etc) }In essence, the ownership model enforces everything needed for consistency at the language level, allowing the memory management system to execute necessary data transfers only, thereby eliminating redundant synchronization operations. \shan{Extending ownership into distributed settings is a contribution for DRust. It might be better to move this after next paragraph when telling about our contributions in DRust. Also the ownership introduction might be a little detailed.. getting a little lost in the big picture.}
% For example, as the simplest case, in figure A(b), after the ownership of data A is transferred from thread 1 on node 1 to thread 2 on node 2, node 2 could directly read data from node 1 without any invalidation operation because it already knows that data A would not be accessed on node 1 because the ownership has been moved from thread 1 on node 1, which is exactly the optimal case.


With this in mind, we propose \tool, a novel language-guided DSM system offering superior performance. The major challenge in designing this system is leveraging the semantic information provided by the ownership model effectively so that the underlying runtime system can execute only the necessary data transfers and synchronization operations while maintaining memory consistency. We designed and implemented corresponding runtime mechanisms for each instruction in the application involving data access right changes, such as reference borrowing, to effectively cache data while maintaining consistency.

Additionally, we enhanced our runtime system with two novel features aimed at improving performance and usability. We introduced a new heap pointer type, allowing programmers to express locality information more effectively and optimize data access patterns, further improving application performance. We also provided a thread scheduler and migrator, offering a seamless way to efficiently distribute a single-machine, multi-threaded application across a distributed system. \shi{We need more elaborations on the contributions of DRust.}

Upon evaluation, our system demonstrated a B$\times$ speedup compared with two baseline DSM systems on five real-world applications. Furthermore, \tool showed a mere Y\% slowdown compared to the optimal performance on a large single machine with sufficient resources.




































% The phenomenon of data explosion has necessitated the distribution of applications across multiple machines. The distribution offers numerous benefits, including enhanced performance, scalability, flexibility, and cost-effectiveness. However, it also introduces a fundamental challenge: ensuring consistency across distributed copies of data. In distributed systems, multiple nodes may hold replicas of the same data, and updates to the data can occur concurrently. Maintaining data consistency necessitates mechanisms to synchronize updates, propagate changes, and ensure that all nodes observe a coherent view of the data. Coordinating these operations in the face of network delays and concurrent access is challenging. It can have a notable impact on system performance. Ensuring data consistency while maximizing performance is a fundamental problem in distributed systems.

% Existing distributed computing systems can be generally categorized into two data access models: the bulk data processing model and the fine-grained data access model. 
% The bulk data processing model is exemplified by frameworks like Spark or Hadoop, which provide a high-level programming model for manipulating large-scale data through transformations and actions. For example, Spark's Resilient Distributed Datasets (RDDs) allow parallel processing of distributed collections across a cluster of machines. However, RDDs have limitations in terms of their generality, as they offer a restricted set of operations for manipulating distributed data. While they excel at coarse-grained data processing tasks, they may not be suitable for more complex data manipulation scenarios. \shan{do we need to add one or two concrete examples that the programming model for coarse-grained data access is hard to support?} \shi{Do we really need to mention Spark in this paper? The rest of the paper is isolated from it, as all other works are fine-grained access systems. And the only downside for this model we gave is a general term "limited programmability". (or we have experiments to show this?) Also, Spark feels like another framework to disable data sharing.}
% On the other hand, fine-grained data access models, such as distributed shared memory (DSM), enable developers to access shared memory across multiple nodes in a distributed system at the object level. DSM provides a programming abstraction that resembles programming on a single machine. However, achieving fine-grained data access in a distributed environment introduces performance challenges due to the necessary synchronization and consistency mechanisms. Coordinating access to shared memory across distributed nodes in the underlying system incurs overhead that can impact overall performance.
% \shan{It might be a little unclear how the two different data access models related to the problem stated in paragraph 1: Ensuring data consistency while maximizing performance}

% In an attempt to achieve fine-grained data access and minimize synchronization overhead in distributed systems, certain programming models have emerged, offering a workaround for the data consistency problem by disabling data sharing. A key exemplar is the actor model, which has been employed in many research studies~\cite{sdsm-atc15,ruan2023nu}. In the actor model, 
% an actor serves as an independent computational entity that encapsulates both state and behavior. Each actor maintains its own isolated state and data, accessing data in other actors solely through message passing. This methodology, while achieving great performance in certain constrained scenarios, is not without its shortcomings.
% In fact, it sacrifices both generality and programming simplicity. 
% Many real-world applications cannot be efficiently implemented within this programming model. Section~\ref{sec:motivation} provides an example illustrating the limitations of the actor model. Even for applications that could potentially fit into the model, it always requires programmers to completely rewrite their applications, which can be a laborious and time-consuming task.
% % an actor is an autonomous computational entity that encapsulates state and behavior. Each actor maintains its own isolated state and data, and accesses data in other actors through message passing. Although this approach achieves performance benefits in certain restricted scenarios, it actually sacrifices generality and programming simplicity. Many real-world applications cannot be (efficiently) implemented in that programming model. An example is shown in section~\ref{sec:motivation}. Even for the applications that could fit into that model, it requires programmers to fully rewrite the applications.

% This paper introduces a novel programming model \tool that offers a solution to the data consistency problem issue intrinsic to distributed systems while providing near-DSM programming simplicity and fine-grained data accessibility. Notably, \tool achieves significantly improved efficiency compared to traditional DSM approaches. The key insight underpinning our design is that most synchronization operations in DSM are superfluous and negatively impact performance. \shan{why or which kinds of most synchronization operations in DSM are superfluous} By leveraging the concept of ownership and incorporating a few simple type annotations, \tool minimizes the need for synchronization operations across servers at runtime, thereby optimizing performance. 
% The idea of ownership has been discussed for many years and gained popularity with the introduction of the Rust programming language. Rust enforces clear rules for ownership, where each value has a single, unique owner at any given time, and the value is automatically destroyed when the owner goes out of scope. Rust also stipulates explicit control over read and write rights to values, allowing either multiple references for reading or a single reference for writing. These rules, enforced during compilation, aim in eliminating data races in single-machine applications.
% The challenge addressed in this paper is how to leverage the concept of ownership to overcome the synchronization overhead problem in DSM. \tool addresses this challenge by tackling three key issues which are illustrated below.
% % This paper presents a general efficient programming model \tool that fundamentally solves the data consistency problem. It has near-DSM programming simplicity and fine-grained distributed data accessibility but with significantly improved efficiency. The key insight behind our design is that most synchronization in DSM is not necessary and greatly hurts performance. By adopting the concept of ownership together with few simple annotations, \tool greatly reduces the number of necessary synchronizing operations across servers and only executes them during runtime. The concept of ownership has been proposed and discussed for many years and becomes much more popular after Rust came out, which is the first practical language that creates clear rules for ownership. In rust, each value has a single, unique owner at any given time. When the owner goes out of scope, the value is automatically destroyed. It also has clear right control over read/write rights to every value: at any time either multiple references can be used to read data only, or only one reference can be used to write to the data. This rule is enforced during compilation time and helps eliminate data races on a single-machine application. The problem now is how can we use the concept of ownership to solve the synchronization overhead problem in DSM. \tool solves this problem by overcoming three challenges.


% Firstly, \textbf{when should synchronizations occur?} 
% Traditional distributed shared memory enforces synchronization after each data mutation when copies of the same data exist on different nodes. This active synchronization, however, leads to significant overhead. On careful observation, we discerned that the rule governed by the concept of ownership -- specifically, allowing either multiple readers or a single writer -- is extremely beneficial in a distributed context. Contrary to the practice of active synchronization post every data mutation, synchronization is only necessitated when the write access alters between references, whether through ownership transfer or mutable reference borrowing. As long as a single reference retains the write access to the data, additional synchronization becomes redundant since no other reference can read or write this data -- a constraint guaranteed by the compiler. In such scenarios, \tool ensures the existence of a solitary data copy. When the write access shifts from one reference to another on a separate node (e.g., during an ownership transfer), and right before the new reference accesses data, the data is migrated from its original location to the server hosting the new reference. Thus, rather than mandating active synchronization following each data mutation, \tool merely requires lazy data migration when the write access changes -- a feature that drastically reduces overhead. In cases where multiple references possess read access to the same data, each of them can freely cache data copies and access them. No synchronization is required in this context, as no reference is permitted to write to the data. We delve into these details in section~\ref{sec:lang}.
% % In traditional distributed systems, when there are copies of the same data on different nodes, if one copy is mutated on one server, it needs to actively synchronize this mutation to other nodes that have this copy, which causes a lot of overhead. But we found that the rule of either multiple readers or one writer enforced by the concept of ownership is very useful in the distributed setting. Instead of actively synchronizing after every mutation of data, synchronization only needs to happen when the writing right changes (either through ownership transfer or mutable references). As long as one reference holds the writing right to the data, synchronization is unnecessary because no one else can read or write this data, which is guaranteed by the compiler. \tool guarantees that in this scenario only one copy of the data exists. When the writing right is transferred from one reference to another reference on another node(e.g. ownership transfer), and the new reference wants to access the data, the data is migrated from its original address to the server where the new reference resides. Instead of doing active synchronization after every mutation to the data, \tool requires lazy data movement only when the writing right of the data changes, which significantly reduces overhead. When there are multiple references with read rights to the same data, all of them can freely cache copies of the data and access them, and no synchronization is required because no one can write to the data now. Details are discussed in section~\ref{sec:lang}.

% Secondly, \textbf{at what granularity should synchronization occur?} 
% As previously discussed, \tool performs synchronization (or, more specifically, data movement) when a new reference possessing write access seeks to access data situated on a different physical node. This reference may hold write accessing rights to a chain of objects, potentially requiring access to a subset of them in the near future. It is apparent that batching this movement is far more efficient than migrating each object individually. However, identifying the optimal granularity for this operation is a non-trivial challenge. We can't simply move all objects together, as this approach is overly coarse-grained and could result in massive useless data transfers, ruining all performance benefits.
% \tool addresses this issue by introducing two type annotations for heap references, allowing programmers to control the synchronization granularity. These annotations enable programmers to define which data should be migrated together (via tie-typed annotations) and which data should be treated separately (via disjoint-typed annotations). We discuss these type annotations in more detail in section~\ref{sec:annotation}.
% % As discussed above, \tool executes synchronization(or more specifically, data movement) happens when a new reference that has the writing right wants to access the data that is on another physical node. The reference could possess writing rights to a chain of objects, and possibly access a portion of them in the near future. Batching the movement is clearly a lot more efficient than moving each object one by one. But determining the optimal granularity is challenging, because we cannot just move all of those objects together which is too coarse-grained and could be very huge. \tool solves this problem by provide two type annotations to heap references, allowing programmers to control the synchronization granularity. Programmers can easily define what data should be brought in together through tie-typed annotations and what data could be placed separately through disjoint-typed annotations. Details can be found in section~\ref{sec:annotation}.

% Thirdly, \textbf{how can we minimize necessary synchronizations?} 
% A synchronization or data movement becomes necessary when the write access is transferred to a new reference on a different physical node. \shi{The introduction of function scheduling here feels a little abrupt. Maybe add one or more sentences at the start. E.g., "In \tool, as in other distributed systems, computation is done in a distributed manner across all participating nodes. Specifically for \tool, a function scheduler sends functions to different nodes for balanced resource utilization."} Instead of scheduling functions to random nodes and subsequently moving data to these nodes, \tool offers programmers a neat abstraction to designate the functions that can be scheduled on another server and to specify the data predominantly accessed by each of these functions. Functions are then scheduled to the node that contains the data being accessed the most, thereby reducing the need for synchronization and optimizing performance.
% % A sychronization or data moving is necessary when the writing right is transferred to a new reference on another physical node. Instead of scheduling functions to a random node and moving data there, \tool chooses to prioritize scheduling functions to near data it accesses the most. It provides programmers with a neat abstraction to specify the functions that could be scheduled to another server and specify the data each of those functions accesses the most. 
% Details are discussed in section~\ref{sec:delegation}.
























% Compute and memory resources are under-utilized in today's datacenters. Prior studies~\cite{legoos-osdi18,patel2015workload} reported low CPU utilization using Google's datacenter traces, showing CPU utilization between 28\% and 56\%, and memory utilization between 40\% to 60\%. This is because the current state of cloud computing, often referred to as Infrastructure as a Service (IaaS), operates on a model where users are provided with pre-defined VM sizes, regardless of whether they fully utilize the allocated resources. This can lead to inefficient resource utilization. Users need to overprovision a larger VM size than necessary to meet their peak demand, resulting in wasted resources during periods of lower utilization. The IaaS model also imposes scalability challenges for single applications: While IaaS provides scalability at the infrastructure level, scaling individual applications within the infrastructure can be challenging. Scaling single applications across multiple VMs can introduce communication overhead and performance bottlenecks. Ensuring efficient communication and synchronization between instances becomes crucial but may not always be straightforward.

% \MyPara{State of the Art}
% To achieve more efficient resource utilization and provide improved scalability for individual applications, new programming models such as the serverless computing~\cite{hellerstein2018serverless} framework and compute-delegation-based systems~\cite{ruan2023nu,nelson-atc15,charles-oopsla05} are proposed. Those techniques require programmers to fully rewrite existing single-machine applications into significantly different programming models. However, many kinds of applications are hard to implement in those models or even if they can, they have to be implemented in a way that would incur heavy communication costs. For the serverless model, programmers separate applications into stateless modules. Different modules can call each other through RPCs. But many applications including some long-running big data tasks (e.g. matrix multiplication) actually cannot be efficiently implemented in the serverless model. Nu~\cite{ruan2023nu}, the current state-of-the-art of compute-delegation-based systems, proposed a new program abstraction called proclet: a lightweight, isolated execution environment that can be created and destroyed on demand. Programmers also define compute functions on top of each proclet. Each proclet has its own heap and prohibits direct data access from other proclets. Instead, they transfer data through RPCs by delegating heap access operations to other proclets. Proclets can be migrated between physical machines as a whole. However, since each proclet has its own heap, they cannot adjust the data layout efficiently when the application's access behavior changes, which leads to too much communication overhead for many real-world complex applications.

% Memory disaggregation, a technique that allows for the separation of memory and compute resources, is another trend in both academia and industry to increase resource utilization in datacenters and improve application scalability. It enables applications to seemingly have a view of unlimited memory, and existing single-machine applications can run on those systems without modification or only with some simple annotations. Current memory-disaggregated systems manage the small local memory as a cache for remote memory. Directly running applications on disaggregated-memory systems extremely sacrifice performance because accessing data on remote servers is orders of magnitude slower than accessing data in local memory. Many kernel techniques, such as~\cite{infiniswap-nsdi17,leap-atc20,fastswap-eurosys20,wang2023canvas,qiao2023hermit}, are developed to improve application data locality, so as to improve application performance. But due to the lack of application semantics, their policy decisions are often incorrect in many cases, highly limiting performance improvement. Some other techniques such as~\cite{ruan2020aifm} choose to delegate some user-defined computation to the remote memory side so as to improve data locality, but this approach brings its own data coherence challenge. Since it also builds on the cache design, programmers can easily trigger data inconsistency issues if they write code where functions executed on the local CPU server modified the data copy in local memory but have not flushed the dirty copy to remote memory while functions executed on remote servers later attempt to modify the other copy of the same data in remote memory. This could lead to application crashes or undesirable results.

% The approaches above strive to improve resource utilization and scalability, while at the same time trying to maintain good application performance either through moving hot data near compute or moving compute near data. But their performance improvement is very limited on many kinds of applications. The key reason is that they are all in lack of a way to define both the data locality relationship and the compute-data relationship. In this paper, we propose \tool, a data-compute-relationship-aware language-system co-design that enables both locality-aware data movement and non-data-race compute delegation. With \tool, programmers are able to define several data units with some simple annotations. The data in the same data unit is always co-located in the same physical server. Programmers can also assign functions to different data units with a simple annotation, and the underlying system will delegate the function execution to the physical server hosting the data unit. Our language design also guarantees that there is no data inconsistency during the compute-delegation process by adopting the ownership concept in Rust~\cite{rust}. \tool aims to provide a more efficient, safer and developer-friendly solution for distributed systems, and to achieve this, \tool must overcome two challenges.

% First, \textit{How to let users define data units in an expressive and clean way?} Our intuition here is that heap data that is likely to be accessed together is usually in the same data structure and connected through references. \tool enables programmers to annotate heap references with two type annotations: \textbf{tie} and \textbf{disjoint}, to specify the intended location of the data pointed by the reference. Heap data connected through tie-typed references consists of one data unit and should always stay on the same physical server. Data connected through disjoint-typed references is not necessarily on the same physical server. Explicit conversion between tie-type and disjoint-type corresponds to different data movement operations, which will be detailed in section~\ref{sec:lang}.


% Second, \textit{How to delegate compute to another server without causing any data inconsistency?} We achieve this by building \tool on top of Rust, a programming language that prioritizes performance, type safety, and concurrency. Rust's emphasis on memory safety and prevention of concurrent data races is achieved through its unique ownership feature. In Rust, each value has a single, unique owner at any given time. When the owner goes out of scope, the value is automatically destroyed. By intelligently integrating Rust's ownership feature with our tie/disjoint type design and corresponding operation semantics, \tool can statically check for potential data races between functions delegated to different servers, ensuring that programs passing the compiler check are guaranteed to have no data race. This eliminates the need for dynamic checks, which can add overhead to the application. \tool's type system design will be detailed in~\ref{sec:lang}.





% \MyPara{Is Disabling Data Sharing a Viable Solution?}
% Several DSM systems~\cite{nelson2015latency,ruan2023nu,moritz2018ray} have chosen to eliminate data sharing in their programming models. One such instance is Grappa~\cite{nelson2015latency}, a DSM system specifically crafted for data-intensive applications that omits cache. It does not permit pulling data for computation. Instead, it delegates every data access and computational task to the server where the data is hosted.
% The system Nu~\cite{ruan2023nu} adopts a similar programming model. Within Nu, developers structure an application as a collection of proclets, each of which encapsulates private data and the associated methods. A proclet is restricted to accessing only its own private data. Like Grappa, if it requires data from other proclets, it must perform a Remote Procedure Call (RPC), thereby shipping the access to other proclets which could be situated on a different physical server. 
% However, this approach comes with its own drawbacks -- it sacrifices generality and programming simplicity. In fact, this approach can be perceived as shifting the responsibility of maintaining data consistency from the system to the programmers themselves. Many real-world applications cannot be easily partitioned into a multitude of small proclets with minimal data sharing requirements. Although programmers could program a proclet to cache data from other proclets that it anticipates will be frequently accessed in the near future, this comes with its own complications. On one hand, an abundance of RPCs could impose significant performance overhead. On the other hand, it demands that programmers explicitly maintain data consistency themselves once their cached data has been altered. This can be a labor-intensive, error-prone process.
% % However, this method sacrifices generality and programming simplicity. Actually, it can be regarded as offloading the responsibility of maintaining data consistency from the system to programmers. Many real-world applications cannot be simply split into a number of small proclets which barely share data with each other. While programmers themselves can still program the proclet to cache the data in other proclets it will potentially be frequently accessed in the near future for potentially better performance through a number of RPCs, on one hand, a lot of RPCs could cause notable performance overhead, on the other hand, it also requires programmers to explicitly maintain the data consistency by themselves once its cached data has been changed, which requires a huge effort and can be error-prone.
% Figure Y illustrates an example of this issue. A naive implementation of the KMeans algorithm in Nu exhibits performance degradation when the number of proclets increases, highlighting the limitations of this programming model.
% % Figure Y illustrates an example of this problem, a naive implementation of KMeans in Nu exhibits performance degradation when the number of proclets increases. (Another example is dataframe in AIFM?)

% \mhr{Show KMeans in Nu}
% (Another example is dataframe in AIFM? Maybe Show that AIFM easily trigger data inconsistency bugs, but our type system can easily check that during the compilation phase?)
% % \mhr{Show Grappa's bad performance shown in Concordia}


==> deprecated/language.tex <==
\section{Language Extension\label{sec:lang}}


This section details \tool's new type qualifiers introduced in \tool for Rust programming language, including explanations of their meanings and guidance on their usage for managing the location of data and computation.
    
\subsection{Type Annotations \label{sec:annotation}}

% As with Rust, programmers need to be aware of the difference between stack values and heap values when programming in \tool. Stack values all have a known, fixed size. Data with an unknown size at compile time must be stored on the heap. We need to follow a pointer to access data in the heap. \tool follows Rust's representation of heap pointers, whose type is written as $Box\langle T\rangle$.
As with Rust, \tool requires programmers to understand the distinction between stack and heap values. Stack values have a definite, fixed size, while data of unknown size at compile-time must be stored on the heap and accessed via a pointer. \tool adheres to Rust's representation of heap pointers, indicated by the type $Box\langle T\rangle$.

The type of each value in the program consists a base value type and a placement annotation. Stack values are annotated as either local ($@l$) or remote ($@r$), while heap values are annotated as local ($@l$), remote ($@r$), or regular (default).
% Each stack value in the program has a local or remote annotation, while each heap value has a local, remote, or regular annotation. Local types are annotated with $@l$; Remote types are annotated with $@r$; Regular types have no annotation, which means it is the default. 
% The placement annotation enables programmers to specify the placement of different data. Local-typed data resides in local memory on the CPU server; Remote-typed data is stored in remote memory servers; Regular-typed data is managed by swap system in the kernel and could be either local or remote during the execution of the application. Note that in real programs, only heap references need to be explicitly annotated. The placement annotation for each stack variable could be directly inferred from the type of function it is in. As for heap values that are not references, their placement annotation could be inferred through their belonging structs.
This placement annotation allows programmers to specify the location of data. Local-typed data resides in local memory on the CPU server, remote-typed data is stored on remote memory servers, and regular-typed data is managed by the swap system in the kernel and may be either local or remote during program execution. Note that only heap references require explicit annotation; the placement of stack variables is inferred based on the type of the containing function, and the placement of heap values that are not references can be determined by their belonging structs.

% Programmers can assign values with different placement annotations (but the same base value type) to each other. A piece of example code is shown below. In the following code, $a1$ stores data in the local stack, while $b1$, $b2$, and $b3$ are local variables storing references to local heap and remote heap. We can assign values between them and corresponding data would be moved from the source value to the destination value.
Programmers can assign values between types with different placement annotations, as long as they have the same base value type. The following code serves as an example. The local variable $a1$ stores data on the local stack, while $b1$, $b2$, and $b3$ are local variables that store references to data on both the local and remote heap. Values can be assigned between them, causing the underlying data to be transferred from the source to the destination. 

\begin{lstlisting}[language=Rust, style=boxed]
// This function is executed on the local CPU server.
fn main() {
    // a1 is stored in local stack by default
    let mut a1: A = ...;
    // b1, b2, b3 are all heap references
    let mut b1: Box<A@l> = ...;
    let mut b2: Box<A@r> = ...;
    let mut b3: Box<A> = ...;

    *b1 = *b2;
    *b2 = *b3;
    *b3 = *b1;
    *b2 = a1;
    a1 = *b2;
}
\end{lstlisting}

\subsection{Struct Definition}

% \tool's type qualifiers can be applied to both primitive types and structs. But inside a struct, there is another type qualifier $@t$ to annotate heap references. It means the data pointed by this reference is of the same placement type with and always stays together with the struct instance containing this reference. The data is called tie-typed data. An example is shown below. The reference $a$ points to a struct instance of type $A$ residing in local memory. The reference field $b1$ inside that instance points to another struct instance of type $B$ which also stays in local memory before line 8. After executing line 8, the instance of type $A$ is moved to remote memory. The data pointed by $b1$ is also moved to remote memory together.
\tool's type qualifiers can be applied to both primitive types and structs. Within structs, an additional type qualifier, $@t$, annotates heap references and indicates that the data referred to is tied to the struct instance and always located in the same server as the struct. This type of data is referred to as "tie-typed data." An example is provided below. The reference $a$ points to a struct instance of type $A$ located in local memory. The reference field $b1$ within that instance points to another struct instance of type $B$ also in local memory, until line 8. After line 8, the type $A$ instance is moved to remote memory, causing the data referred to by $b1$ to be moved there as well.

\begin{lstlisting}[language=Rust, style=boxed]
struct A {
	b1: Box<B@t>,
	b2: B,
	b3: &B
}

let a: Box<A@l> = ...;
let mut b: Box<A@r> = a;
\end{lstlisting}


\subsection{Object Creation}

There are three functions for allocating heap data

\begin{itemize}
    \item \textbf{new} is the default keyword for creating objects and allocates general-typed data on the local heap.
    \item \textbf{lnew} allocates local-typed data on the local heap.
    \item \textbf{rnew} allocates remote-typed data directly on the remote memory server's heap.
\end{itemize}

\begin{lstlisting}[language=Rust, style=boxed]
let mut a2: Box<A> = Box::new(A{field1: 0, field2: 0});
let mut a2: Box<A@l> = Box::lnew(A{field1: 0, field2: 0});
let mut a2: Box<A@r> = Box::rnew(A{field1: 0, field2: 0});
\end{lstlisting}

\subsection{Remote Functions}

% When programming using \tool, programmers need to specify what functions they want to offload to the remote side. This is achieved through function annotations. All functions that need to be offloaded should be annotated with $@remote$. Functions without annotations are regular functions and are executed in the local CPU server. Remote functions can only dereference and access remote-typed data. Regular functions can dereference local-typed data and regular-typed data, while local functions can also dereference remote-typed data in value-assigning statements because the nature of those statements is moving data through RDMA operations.
In \tool programming, function offloading to the remote side is specified through annotations. Functions to be offloaded must be annotated with $@remote$. Functions without annotations are executed locally on the CPU server. Remote functions can only access remote-typed data, while regular functions can access both local and regular-typed data. Local functions can also access remote-typed data in value-assigning statements for moving data through RDMA operations.

\subsection{References and Borrowing}

% In \tool, all placement type conversion (data movement) can only be done through ownership transfer instead of reference value copying. For example, in the following code, line 4 is forbidden because we cannot assign a reference values to another one with different placement types. Line 5 is also not allowed because in rust, we cannot move a value from its owner when it is borrowed by another reference. But line 8 is allowed since at that time, $b$ has gone out of scope and does not exist. 
In \tool, conversion between different placement types is achieved through ownership transfer, not reference value copying. For example, in code, line 5 is prohibited as it tries to assign a reference value to another with a different placement type. Line 6 is also not allowed because in Rust, a value cannot be moved from its owner while it's borrowed by another reference. However, line 8 is permitted as at that point, the reference $b$ is out of scope and no longer exists.

\begin{lstlisting}[language=Rust, style=boxed]
let mut a: Box<A@l> = Box::lnew(A{...});
{
    let mut b: &(A@l) = &mut (*a);
    // The following operations are forbbiden
    // let mut c: &(A@r) = b;
    // let mut a1: Box<A@r> = a;
}
let mut a1: Box<A@r> = a;
\end{lstlisting}

% \tool's type qualifier $@t$ is special. For simplicity, we do not allow borrowing data owned by heap reference with that annotation. For example, the following code is not allowed and could not pass the compiler's type check. We made this design choice mainly to avoid the dangling pointer problem. If we allow creating reference to tie-typed data, then after moving the instance containing its owner, it also needs to be moved. The original reference now becomes dangling pointer and points to meaningless data.
In \tool, the $@t$ type qualifier requires special handling. To simplify programming, borrowing of data owned by a heap reference with this annotation is not allowed. This design decision is made mainly to prevent the risk of dangling pointers. The data would need to be moved along with its owner instance when the instance is moved. If creating a reference to tie-typed data was allowed, the original reference would then become a dangling pointer, pointing to meaningless data. For this reason, code such as the following is not permitted by the compiler's type check.

\begin{lstlisting}[language=Rust, style=boxed]
struct A {
	b1: Box<B@t>,
	b2: B,
	b3: &B
}

let a: Box<A@l> = ...;
let mut b = &mut *(a.b1);
\end{lstlisting}

==> deprecated/method_dep.tex <==
\section{Design\label{sec:lang}}


\subsection{Data Management \label{sec:annotation}}

As introduced in section~\ref{sec:intro}, the biggest challenge in designing the language is how to provide programmers with an expressive but also clean way to define data locality relationships. \tool is built on top of Rust. In Rust, heap-allocated data is managed through references called $Box\langle T\rangle$, which represents a unique owned pointer to a heap-allocated value of type T. Each heap-allocated data in Rust have one and only one owner. This unique ownership implies that the instance graph structure is actually a forest (a collection of disjoint trees). And this structure naturally becomes a good choice for defining the data locality relationship. After accessing the owner, applications are more likely to access data owned by it, and vice versa. However, naively employing ownership as the only way to define the data relationship and co-locating all data that has the same ancestor is too coarse-grained. For example, a hashmap could be too huge to fit into any physical machine. So programmers must have a more fine-grained way to express the data locality semantics of their applications. 

\begin{figure}
\centering
\begin{tabular}{c}
\includegraphics[width=\linewidth]{figs/Before.pdf} \\
(a) Before type conversion\\
\includegraphics[width=\linewidth]{figs/After.pdf} \\
(b) After type conversion
\end{tabular}
\caption{\label{fig:example_types} Tie-typed data always stay on the same physical server as its owning reference.}
%   \vspace{-1em}
\end{figure}


\tool achieves that by providing two type annotations: \textbf{tie} and \textbf{disjoint}. The type of each heap reference in the program consists of a base type $Box\langle T\rangle$ and a placement annotation suffix $t$ or $d$. This placement annotation suffix allows programmers to specify the intended locality relationship of data. Heap data owned by tie-typed references\footnote{We call heap references of type $Box_t\langle T\rangle$ as tie-typed references and heap references of type $Box_d\langle T\rangle$ as disjoint-typed references.} is guaranteed to reside in the same physical server as the reference itself, while there is no such guarantee for disjoint-typed data\footnote{Heap data owned by tie-typed/disjoint-typed references is called tie-typed/disjoint-typed data.}. Figure~\ref{fig:example_types} shows an example instance graph of a \tool program. Each dashed arrow represents a disjoint-typed reference and each solid arrow represents a tie-typed reference. Heap data owned by tie-typed reference always stay together with the instance containing its owning reference. For example, instance A and instance B are guaranteed to stay on the same physical server. As for data owned by disjoint-typed references like instance D, it could but not necessarily be placed onto another different server from instance A, which all depends on the runtime scheduler which will be detailed in section~\ref{sec:sys}.

However, the optimal data placement is usually not static during the execution of applications. \tool enables programmers to reorganize the data by doing explicit type conversion between tie-typed and disjoint-typed references. Programmers can assign references between types with different placement annotations, as long as they have the same base type. Assigning a disjoint-typed reference to tie-typed reference by doing explicit type conversion corresponds to data movement between physical servers, which is done by underlying runtime system. For example, shown in listing~\ref{list:annot} and figure~\ref{fig:example_types} (a), there are different instances with different types. And in this example, there is a function \textit{move} that is going to be executed on server 1. Stack variable $d$ is a tie-typed reference pointing to instance $D$. $D$ is of type Dstruct and has two tie-typed reference fields: one pointing to instance $E_0$ of type Estruct and one pointing to instance $F$ of type Fstruct. F has one disjoint-typed reference field pointing to instance $E_1$ which is also of type Estruct but resides on server 2. After the function \textit{move} starts, as shown in line 17, it first explicitly convert the disjoint-typed reference $d.f.e$ to a tie-typed reference and move it into newly created stack variable $tieE$. And then it moves the reference stored in $tieE$ to $d.e$, shown in line 18. New data placement after the function finishes is shown in figure~\ref{fig:example_types} (b). $E_1$ and $H$ are moved to server 1 because now $D$, $F$, $E_1$ and $H$ become a new data unit. Instance $E_0$ is dropped.


% \begin{figure}
\begin{lstlisting}[language=Rust, style=boxed, basicstyle=\small, label=list:annot, caption=Type annotations and explicit type conversion.]
struct Dstruct {
    e: TBox<Estruct>,
    f: TBox<Fstruct>,
}

struct Estruct {
    h: Option<TBox<Hstruct>>,
    i: Option<DBox<Istruct>>,
}

struct Fstruct {
    e: DBox<Estruct>,
}

// This function is executed on server #1
fn move(d: TBox<Dstruct>) {
    let tieE: TBox<Estruct> = tie(d.f.e);
    d.e = tieE;
}
\end{lstlisting}
% \caption{}
% \end{figure}

\begin{lstlisting}[language=Rust, style=boxed, basicstyle=\small, label=list:annot, caption=Type annotations and explicit type conversion.]
struct Dstruct {
    e: TBox<Estruct>,
    f: TBox<Fstruct>,
}

struct Estruct {
    value: i32,
    h: Option<TBox<Hstruct>>,
    i: Option<Box<Istruct>>,
}

struct Fstruct {
    e: Box<Estruct>,
}

// This function is executed on server #1
fn move(d: TBox<Dstruct>) {
    let e_value = d.f.e.value; //E1,H moved to server1
    let h_value = d.f.e.h.value;
}
\end{lstlisting}

Because large data structures are always stored in a heap instead of on stack, \tool's annotations only apply to heap references but not stack-allocated data. Each function on each server has its own stack frame and can only access local stack data on its residing server.


\subsection{Compute Delegation \label{sec:delegation}}

\tool is able to delegate compute to different physical servers to achieve better application performance and better compute scalability. \tool provides programmers with a neat way to specify where each function should be executed. Programmers can annotate functions that can be delegated with \textbf{\#[delegate]} and pass it a disjoint-typed heap reference as the first parameter. The function will be executed on the server where the disjoint-typed heap reference points to. For example in listing~\ref{list:delegate}, $rfunc$ is annotated with \textbf{\#[delegate]} and called in the $main$ function. Stack variable $a$ is a disjoint-typed reference and is passed as the first parameter to $rfunc$. \tool's underlying runtime system would schedule that function to the server where $a$ points to, and thus in the body of $rfunc$, $a$ becomes a tie-typed reference. Functions without annotations are always executed on the server where they are called.

\begin{lstlisting}[language=Rust, style=boxed, basicstyle=\small, label=list:delegate, caption=Delegate compute to different physical servers.]
#[delegate]
fn rfunc(a: TBox<A>, b: i32) {
    ...
}

fn main() {
    let a: DBox<A> = DBox::new(...);
    rfunc(a, 0);
}
\end{lstlisting}


\begin{figure}
\centering
\includegraphics[width=\linewidth]{figs/sys_overview.pdf} 
\caption{\label{fig:sys_overview} System Architecture Overview.}
\end{figure}



\tool's underlying runtime system enables programs written in \tool language to efficiently and safely run in a distributed environment. An overview of the system architecture is shown in figure~\ref{fig:sys_overview}. Programmers write a program that contains data units and functions that operate on data units. The underlying resource manager monitors all physical resources on each server, and schedules data units and functions to servers. It considers load balancing and resource utilization when doing data unit scheduling but always schedules functions to the server holding the data unit specified by the programmers through function parameters. 

\begin{figure*}
\centering
\includegraphics[width=.9\linewidth]{figs/manager.pdf}
\caption{\label{fig:workflow} Workflow of \tool's underlying runtime system. }
%   \vspace{-1em}
\end{figure*}

\begin{lstlisting}[language=Rust, style=boxed, basicstyle=\small, label=list:workflow, caption=Workflow example code.]
#[delegate]
fn B(d2: TBox<T2>) {
    let d3: TBox<T3> = tie(d2.f);
    process(d3);
    let d4: DBox<T4> = DBox::new(...);
}

fn A() {
    let d1: TBox<T1> = initialize();
    B(d1.f);
}
\end{lstlisting}
% let d3: DBox<T3> = DBox::new(...);
% let d2: DBox<T2> = DBox::new(T2{f: d3, ...});
% let d1: TBox<T1> = TBox::new(T1{f: d2, ...});

A more concrete and complete example showing how the underlying runtime system works is illustrated in figure~\ref{fig:workflow} and listing~\ref{list:workflow}. In this example, function A is started on server 1 and it first initialized data units 1, 2, and 3. It stores the tie-typed reference to data 1 in the stack variable $d1$. Data unit 1 contains a disjoint-typed reference field $f$ pointing to data unit 2, and data unit 2 contains a disjoint-typed reference to data unit 3. After initialization, function A calls function B and input $d1.f$ as the first parameter, meaning function B should be delegated to the server holding data unit referenced by $d1.f$. Therefore, the underlying system schedules function B to server 3 (step \textcircled{0}) and moves the ownership of data unit 2 from $d1.f$ (step \textcircled{1}) to the function parameter $d2$ stored in function B's stack (step \textcircled{2}). After that, in line 3, function B explicitly converts the disjoint-typed reference $d2.f$ to a tie-typed reference and moves it to a stack variable $d3$. Correspondingly, the underlying system moves the data unit 3 from server 2 to server 3 (step \textcircled{3} and \textcircled{4}), and also informs the global resource manager that the memory occupied by the old data unit 3 on server 2 could be reclaimed now (step \textcircled{5}). At the end of function B, programmers create a new disjoint-typed instance by calling the built-in function \textit{DBox::new}. That runtime function firstly consults the resource manager where to put the new instance (step \textcircled{6}) and then creates an instance at the target server and returns a disjoint-typed reference (step \textcircled{7}). Note that in \tool's implementation, it does not consult the resource manager every time it asks for or release some resource, which is inefficient. Instead, it maintains a buffer on each server and will allocate resource from or release resource to the buffer. When the buffer is too small or too big, the underlying runtime will ask for more from or release some resource to the global resource manager.


\section{Data Consistency}

The problem of data consistency in distributed systems has been a significant challenge for a long time. In a distributed system, functions executed on one server often need to access data hosted by other servers. However, synchronizing every remote data access is impractical due to the excessive communication overhead it incurs. Each server usually needs to cache certain data hosted by other servers to improve performance. However, when the program modifies cached data but does not carefully synchronize it with other servers, and then another function accesses the original data, data inconsistency issues arise.

To address this problem, existing systems like Nu and Ray impose system-level restrictions on programmers. Nu mandates that functions within each "proclet" can only access data residing in the current proclet's heap. Consequently, every access to other proclets' data requires executing a Remote Procedure Call (RPC), which can easily become a performance bottleneck. On the other hand, Ray takes a different approach by enabling all functions on all servers to access data in its object store system, but with the constraint that all data in the object store is immutable. Modified objects must be stored as new objects in the object store to be accessed by other functions, resulting in significant resource waste.

In contrast, by guaranteeing data consistency at the language level, our solution enables programmers to flexibly move data between servers to mitigate high communication overhead without causing big memory resource waste. In \tool language, we enforce a rule that every program can only dereference tie-typed references. Programs that fail to comply with this rule cannot be compiled. This rule ensures that in a valid program, every function can only access data residing in the current server where it is executed. Whenever functions on another server need to access it, a synchronization operation is enforced by the language. The synchronization is explicit to programmers, avoiding potential hard-to-find performance bugs.

But how does \tool guarantee data consistency at the language level as well as provide great performance? We illustrate this by first showing why pure Rust does not work and then why \tool's language extension makes it possible. It is known that safe Rust programs have a data-race-free guarantee. However, as shown above, naively running Rust programs on a cacheable distributed system might still cause the same data inconsistency problems without careful synchronization. The key problem here is that there could be two copies of the same data on different servers at the same time. Strawman solutions to this problem including prohibiting data movement and prohibiting data mutability, all of which have limitations shown above. So the key solution here is that as long as we can guarantee there is only one copy for each data on every server, the problem is solved. Thanks to Rust's ownership feature, this could be easily achieved. A strawman solution in Rust is to move data to local memory every time dereferencing the heap reference. But it requires a runtime check for every heap access and frequent data fetching from remote servers, badly harming performance. Another possible strawman solution in Rust is when dereferencing the heap reference, we can move all data either directly or indirectly owned by the reference to local memory. But it clearly also does not work because it is too coarse-grained and restricts scalability. If the data size is too big, then it cannot fit into a single-machine memory at all. Luckily, \tool's language extension with \textbf{disjoint} annotation to heap references allows programmers to control this in fine granularity. Programmers can easily define what data should be brought in together and what data could be placed separately. In this way, \tool enables both data-consistency and great performance and scalability.


\section{Borrowing Values}

\mhr{TODO: rename heap reference above to heap pointers}

\mhr{TODO: basic idea: We enable two copies of a single data for value borrowing. Each reference also have two types: tie-typed and disjoint-typed. When doing conversion from disjoint-typed reference to tie-typed reference, we direct copy data to local memory without destroying data and releasing resources on other servers. When the function exits (reference goes out of scope), local data copy referenced by tie-typed immutable references is directly discarded, and local data copy referenced by tie-typed mutable references will be first written back to the original data location and then discarded. This would not break the data-consistency rule in \tool, though with copies.}


% Data access through immutable reference is the most complicated case. Unlike the owner or the mutable reference which has exclusive access right to the data so that they can freely move data without concerning about concurrency and consistency problem. There can be multiple immutable references pointing to the same data. But the good thing is that the ownership model guarantees that all references can only read data instead of write to it, which makes the whole process for maintaining consistency much simpler. The immutable reference also records two addresses: one for data address but the other one for the original address of the data. When a thread would like to access the data through an immutable reference, \tool also firstly checks the data address and directly access it if it is in local memory. If the data is on a remote server, as depicted in figure~\ref{fig:immutable}, \tool copies the object to local memory address $p$ (\textcircled{1}), and updates the immutable reference's data address to let it point to the new address $p$ (\textcircled{2}). But it will not deallocate the original data on the remote server. However, it needs to execute another additional operation, which is inserting/updating an entry in a local hashmap which is mainly for maintaining cache copies. There is a hashmap on each server, the key in this hashmap is the original address of data, and the value entry is a pair of the data copy address on this server and how many immutable references currently points to it. So after updating the immutable reference, it needs to insert an entry to the local hashmap meaning that the local server contains a cache copy of data object $A$ and one reference is pointing to it. Then when another thread also want to access the same data object through another immutable reference, it can firstly check the hashtable if the current server contains the cache copy of the data to be accessed, if yes, then it increase the second value of the value entry and updates the immutable reference with the first value of the value entry, and access it. This process is just like a cache hit operation. Then when immutable references go out of scope, \tool decreases the count value in the value entry in the hashmap, and when the count is 0, the data object $A$ is dropped by \tool. 
% The whole process only incurs one network trip to fetch the data when a server firstly accesses a data object. So no synchronization overhead over network is added, only local synchronization overhead exists.\



% Special treatment is also need when creating new shared immutable references by copying from existing references and dropping references when they go out of scope.
% When copying shared references, only the original data address will be copied, leaving local copy field of the new reference as null. This is for maintaining the correctness of the reference count in the hashmap and guarantee the local copy address is indeed local. When the program accesses data through the new reference next time, \tool will follow the procedure above to update the local copy field and the hashmap.
% As for the scenario when an immutable reference goes out of scope, \tool needs to decrement the hashmap's reference count if its local copy field is not null. Once this count reaches zero, indicating no active references, \tool deallocates the local data copy.


% To prove sequential consistency for \tool, we need to prove the latest write visibility property for \tool, i.e. once a write operation is performed, any subsequent read operations (from any processor) should see that write, as long as no other writes to the same location have intervened.
% First, Rust's ownership model guarantees only one writer can update a memory location at a time, so it ensures that the writing memory operations to the same memory location are perceived to be executed in a sequential order. All reads to the same memory location can only happen between two adjacent writing operations and reflect latest writing operation. \tool preserves this property. 
% Second, though multiple data copies can be cached in different servers through immutable references in \tool, \tool guarantees that there only exists a single data copy when the program is writing to it (via owner or mutable references). So anytime the program is writing a data, there is no other data copies. All subsequent reads to this data before the next write operation must all either directly read from this only one copy, or duplicate data from this copy. So they always read value of the last write operations. 
% Programs involving unsafe code, mutexes and atomics would be more complicated. We discuss mutexes and atomics in section~\ref{sec:std}, and unsafe code in section~\ref{sec:unsafe}.
% Given that safe Rust inherently prevents data races, \tool extends this guarantee to distributed shared memory environments, ensuring sequential consistency as long as the program is written with safe Rust code. Rust's ownership model guarantees exactly one writer can update a memory location at a time, so it ensures that the writing memory operations to the same memory location are perceived to be executed in a sequential order. And all reads to the same memory location can only happen between two adjacent writing operations and gets the value of the previous writing operation. \tool would not change Rust's program execution order. We only need to prove the latest write visibility for \tool, i.e. once a write operation is performed, any subsequent read operations (from any processor) should see that write, as long as no other writes to the same location have intervened. Though multiple data copies can be cached in different servers through immutable references in \tool, \tool guarantees that there only exists a single data copy when the program is writing to it (via owner or mutable references). All subsequent reads must all either directly read from this only one copy, or duplicate data from this copy, so that they always read the most recent value. So \tool also offers sequential consistency for data-race-free programs.
% The approach to handling unsafe code, which introduces additional complexity to maintaining this consistency model, is discussed in detail in section~\ref{sec:unsafe}.

% \subsubsection{Data-data Locality\label{sec:tbox}}

% \begin{figure}
% \begin{lstlisting}[language=Rust, style=boxed]
% struct Dstruct {
%     e: TBox<Estruct>,
%     f: TBox<Fstruct>,
% }
% struct Estruct {
%     h: Option<TBox<Hstruct>>,
%     i: Option<Box<Istruct>>,
% }
% struct Fstruct {
%     e: Box<Estruct>,
% }
% // This function is executed on server #1
% fn access(d: TBox<Dstruct>) {
%     let e_value = d.f.e.value; //E1, H moved to server 1
%     let h_value = d.f.e.h.value; 
% }
% \end{lstlisting}
% \caption{Code example of TBox pointers. \label{lst:tboxpointer}}
% \end{figure}



% As shown in section~\ref{sec:runtime}, each memory access in \tool involves a local runtime check to determine whether the access is in local memory. Though this operation is executed locally and requires no network operations involving other serves, when the workload is very memory intensive, which will be shown in our evaluation drill-down, this check can also incur relatively visible overhead. 
% Besides, if certain objects are usually accessed together, many of those objects can actually be fetched together to improve overall network throughput instead of fetching them one by one when accessing them. For example, \mhr{Think of an example use case here.}
% To overcome these two problems, we propose a new language construct: Tie-typed Heap Pointer $TBox<T>$, in comparison with Rust's conventional heap pointer $Box<T>$. Its usage is the same as $Box$, but there are two additional embedded semantics inside this language construct: (1) The owner points to an object stored in heap memory, and the owner and the object always stays on the same server, so there is no runtime check when accessing the object through the owner because they must be in the same server. (2) When fetching the owner to local memory, the objects that the owner owns through this type will also be fetched together to ensure the previous property and batch the data transferring operations.


% \begin{figure}
%     \centering
%     \begin{tabular}{c}
%         \includegraphics[scale=0.55]{figs/TBoxBefore.pdf}\\
%         (a) \\
%         \includegraphics[scale=0.55]{figs/TboxAfter.pdf}\\
%         (b)
%     \end{tabular}
%     \caption{An example of TBox Pointer. \label{fig:tbox}}
% \end{figure}


% An example is shown in figures~\ref{fig:tbox} and~\ref{lst:tboxpointer}. Objects spread across four servers, and the program is executing an \textit{access} function on server 1. This function firstly accesses object E1 through $d.f.e$. This operation would retrieve object E1 from server 2 first, and then access the value of this object. However, in this case, E1 has a tie-typed heap pointer pointing to object H. So H will also be batch fetched together to server 1. Then when accessing the value of H, there is no need to do any data transferring operations. Besides, when accessing H through $d.f.e.h.value$, it only incurs one runtime check when dereferencing $d.f.e$ because it is a regular Box pointer. But for dereferencing $d$, $d.f$, and $d.f.e.h$, there is no need to do runtime check, because we already know the owner is in local memory, so the objects pointed by the pointer must also be in local memory. If we do not use TBox pointers, then this operation will incur four times runtime check.

% % \subsection{Thread Manager}

% \subsubsection{Data-compute Locality \label{sec:spawnto}}
% \mhr{To update}

% \begin{figure}
% \begin{lstlisting}[language=Rust, style=boxed]
% fn main() {
%     let d: Box<D> = Box::new(D);
%     let d2: Box<D> = Box::new(D);
%     let h = spawn(move || {compute_func(d)});
%     let h2 = spawn_to(d, move || {compute_func(d)});
%     h.join(); h2.join();
% }
% \end{lstlisting}
% \caption{Code example of thread spawning interface. \label{lst:thread}}
% \end{figure}


% \yiying{Right now, this section has nothing to do with Rust and can be applied to any DSM system. What's unique here?}

% In order to help programmers seamlessly distribute a single machine application to multiple servers, we design and develop a thread manager in \tool. \tool's thread manager provides a mostly same interface as Rust's original thread interface to save programmers' effort to learn new interface or modify their existing applications. Programmers can distribute the workload to other servers by spawning new threads. The challenge or we can say the goal of this manager is two fold. First, we want to reduce data transfer between servers, i.e. we want the thread to be scheduled to the server which contains most of the data it is going to access. Second, we want to avoid resource congestion (including both compute congestion and memory congestion), otherwise we can just put all data on the same server and schedule all compute threads to that server. \yiying{What does resource congestion mean? does it mean multiple threads need to use memory/CPU resources and there's only limited?} To achieve this, the thread managers needs to gather semantics from programs about (1) what data it is going to access (2) how much local memory it requires to run the workload. \yiying{should you also consider how much an object is accessed by multiple threads? for example, if two objects have the same size, one is mostly only accessed by thread 1, one mostly accessed by 10 threads. For the latter, you would wnat to schedule the 10 threads together as much ass possible, while for the former, there's no such concern.} The thread manager then monitors the available resources on different servers and intelligently schedule threads to the server with enough resource (compute and memory) and prioritizes the server holding the most data the thread is going to access. To get the first information, we provide an interface to enable programmers express this semantics. Figure~\ref{lst:thread} shows an the example of this interface. \yiying{Should go through the code example or refer to line numbers to explain what's going on. Right now, I don't really know what compute\_func(d) or move mean.} 
% It accepts an additional argument of type Box<T>. It means the new thread it is going to spawn accesses this data structure the most. \yiying{can this be inferred from static analysis?} 
% Then the thread scheduler checks whether the data holding the object pointed by this heap pointer has enough compute resource, if yes, it schedules the thread there. 
% If there is not enough compute resource or the programmers does not provide this information, the scheduler then schedules the thread based on resources. 
% The biggest challenge here is that we would like be able to spawn as many threads as possible and let each thread have enough compute resource and memory resource. 
% It is easy to achieve this for compute resource because we can assume each thread consumes one core and \tool monitors how many cores are available on each machine and schedule the thread to a server with available cores. 
% However, memory is much more complicated. It is difficult to predict how much memory a thread requires and impossible to do optimal scheduling even knowing memory usage information. 
% So here we adopts an adaptive method. When firstly spawning a thread, \tool adopts a common method used in many cloud computing provider companies to schedule VMs among NUMA nodes, which is always schedule the new unit to a place with the most available resources. During the running of the application, we have a online profiler that records how much memory are allocated through this thread. \yiying{need to talk about profiling overhead} This information will be used in our later scheduling decisions. Because a function can be spawned on different threads many times, we assume the memory usage of these threads are similar. \yiying{This assumption is not grounded and should not be true when a program receives different inputs (and for the most cases, a program's executions will have different inputs).} We calculate the moving average of the memory usage of each function that has been spawned before. When the manager is choosing a server to spawn a new thread executing a function that already has history information, it schedules this new thread to a server with available compute and the least but enough memory resource. \mhr{The policy here needs discussion.}

% This scheduling policy works well in our evaluation on three common workloads in data centers. \yiying{did you eval use different inputs?}



% Three primary mechanisms for accessing heap data in rust are through: (1) A singular owner; (2) Mutable Reference (\textit{\&mut T}), offering exclusive but temporary read/write access, reverts the rights to the owner once the reference's scope ends; (3) Immutable Reference (\textit{\&T}), permits temporary and read-only access, where multiple immutable references can exist concurrently, provided no mutable reference is active. 
% % Reference-counting pointers (Arc<T>), permits multiple owners with only read access. 
% Our runtime system's task is to manage these access paradigms, ensuring data consistency with minimal synchronization.

% \subsubsection{Memory Access Handling \label{sec:memory}}

% \tool re-implements the core Rust language constructs (\ie, \codeIn{Box}, \codeIn{\&}, and \codeIn{\&mut}) for transparent support of data distribution and sharing, hiding the complex details of memory allocation/deallocation, moving objects, and coherence maintenance (\S\ref{sec:pa:memory-management}). \tool supports distributed threading and concurrency control by adapting common Rust standard libraries upon the core language constructs (\S\ref{sec:pa:std-lib-support}). Furthermore, \tool offers language construct extensions to allow developers to build more efficient applications with data affinity hints and high-level data structure libraries 

% Like many existing distributed shared memory (DSM) systems~\cite{cai2018efficient, sdsm-atc15, taranov2021corm, wang2021concordia, kaxiras2015turning}, \tool primarily handles heap memory management. This choice ensures that while stack variables remain private to each thread and local to the machine of execution, heap data is distributable across multiple physical servers, accessible to any thread on any node. Figure~\ref{fig:address} illustrates the addressing model and overall design of \tool. In this model, the heap uses the well-established partitioned global address space (PGAS) approach \cite{el2005upc,yelick2007productivity,coarfa2005evaluation}, which conceptually unifies the address space across nodes in a distributed memory system, with each node managing a statically partitioned segment of this global space. \shi{Also talk about the stack address space?}

% \tool's architecture is modular, comprising three core components. The central component is the runtime system, which capitalizes on the ownership semantics inherent in Rust \shi{\sout{- a system programming language that \tool is built upon—to ensure memory consistency with reduced synchronization demands}}. The second component is a novel language construct unique to \tool, designed to empower programmers to enhance performance further. Lastly, a thread management module facilitates the distribution of applications from a single machine across multiple servers. These modules are delineated in the subsections that follow.


% \shi{This paragraph feels abrupt. Why don't we talk about reference cases and then introduce the problem with and the solution with the owner together?} Contrary to initial expectations, data access via ownership is complex, more so than through references. A simplistic handling of owner access might involve verifying the data's location before access: if the data resides in local memory, the runtime performs standard read/write operations; if the data is remote, \tool would transfer the object to local memory and update the owner's pointer. At first glance, this approach seems viable, given the exclusivity guaranteed by the ownership model, ostensibly obviating concerns about consistency and concurrency. However, this view neglects potential complications arising from the coexistence of the owner with immutable references, which may still be active, thus risking the creation of dangling pointers during ownership dereference. Such a conflict could occur if, unknowingly during dereferencing, other references remain linked to the object in question. We will, therefore, explore how our system adeptly manages references and subsequently outline our strategy for handling ownership complexities.

% As discussed in section~\ref{sec:motvation}, in rust, heap data can be accessed in four primary ways: (1) Owner allows exclusive read and write access. Heap-allocated data can be accessed through ownership move from one variable to another. It is enforced that there is only one owner of the data at any given time (2) Mutable Reference (\textit{\&mut T}) also allows exclusive read/write access to the data. Different from owner, the access is temporary. When the reference goes out of scope, the access right goes back to the owner. (3) Immutable Reference (\textit{\&T}) allows temporary and read-only access to the data. Multiple immutable references can coexist simultaneously, but they cannot be used alongside a mutable reference. We now discuss how our underlying runtime system handles the heap data access through these three primary ways and avoid data inconsistency without too many synchronizations.


% Contrary to straightforward intuition that data access through owner should be the simplest case, it is actually more complicated than access through references. A naive way to handle access from owner could be first checking the place of the data to be accessed. If the object to be accessed is in local memory, then our runtime just perform regular read/write access. If the current owner points to an object on a remote server, \tool could move that object to local memory and update the pointer stored in the owner. This looks correct at the first glimpse, since the ownership model guarantees that there is only one owner for each object, so that it is safe for us to move the object and update the owner without need to concern about consistency and concurrency problem. However, this assumption oversimplifies the scenario, because the owner could coexist with immutable references and still be dereferenced to get the object, and during runtime, when we are dereferencing an owner, we can only know the type of this dereferencing operation but cannot know whether other references to the same value also exist at the same time, and if we naively moves value to local memory when dereferencing the owner, it may cause dangling pointer problems for other references. So below we firstly discuss how we handle the references and then discuss how to handle the owner.

% \begin{figure*} [h!]
%     \centering
%     \begin{tabular}{cc}
%     \includegraphics[scale=0.7]{figs/owner.pdf} &
%     \includegraphics[scale=0.7]{figs/mutabler.pdf} \\
%     (a) Owner & (b) Mutable Reference \\\\
%     \multicolumn{2}{c}{\includegraphics[scale=0.5]{figs/immutabler.pdf}}\\
%     \multicolumn{2}{c}{(c) Immutable Reference}\\
%     \end{tabular}
%     \caption{Handling memory access through different ways in \tool \label{fig:runtime}}
  
% \end{figure*}


% \begin{figure}
% \centering
% \includegraphics[scale=0.8]{figs/owner.pdf}
% \caption{Handling memory access through owner \mhr{Will replace the figure with better formats}\label{fig:owner}}
% \end{figure}


\MyPara{Mutable Reference}
Accessing data via a mutable reference ensures exclusivity. Different from Rust, \tool's mutable reference tracks both the data's location and the owner's address. When accessing data through this reference, our tool (\tool) first verifies the data's location. If the data resides locally, it is accessed directly. However, for remote data, as shown in Figure~\ref{fig:mutable}, \tool performs three steps: it relocates the object to local memory address $p$ (\textcircled{1}), reassigns the mutable reference to point to $p$ (\textcircled{2}), and asynchronously requests the remote server to free the previous memory (\textcircled{3}). And when a mutable reference expires, \tool will update the owner with the new address $p$ (\textcircled{4}) before the reference can be safely discarded (\textcircled{5}), ensuring the owner retains access to the most recent data. Our update to the owner will not cause any concurrency issue because the ownership model statically guarantees that no one can access the owner before the mutable reference is dropped.
% Data access through mutable reference is the simplest case, because when there is a mutable reference, it is guaranteed that no one else has the access right to the value. The mutable reference records two addresses: one for data address and one for the owner's address. Each time the program accesses the data through the mutable reference, similar to accessing it through owner, \tool firstly checks the place of the data to be accessed and directly access it if it is in local memory. If the data is on a remote server, as depicted in figure~\ref{fig:mutable}, \tool also firstly moves the object to local memory address $p$ (\textcircled{1}), updates the mutable reference's data address to let it point to the new address $p$ (\textcircled{2}), and sends an asynchronous request to the remote server to deallocate the old memory space (\textcircled{3}). Different from accessing through owner, when the mutable reference goes out of scope, \tool cannot just drop the reference itself, it needs to write the new address $p$ to owner (\textcircled{1}) before dropping itself (\textcircled{2}). Thus after the access right goes back to the owner $O$, the owner can access the latest data through the updated address.



% \subsubsection{Owner}
% \tool firstly checks the place of the data to be accessed. There are two possible scenarios in this case. If the object to be accessed is in local memory, then our runtime just perform regular read/write access. If the current owner points to an object on a remote server, as depicted in figure~\ref{fig:owner}, \tool firstly allocates a new memory space with address $p$, copies the object to local memory $p$ through a one-sided RDMA read operation (\textcircled{1}). After that, it updates the owner to let it point to the new address $p$ (\textcircled{2}). Finally, it sends an asynchronous request to the remote server to deallocate the old memory space occupied by the old object $A$ (\textcircled{3}). 
% Since the ownership model guarantees that there is only one owner for each object and there is no other reference can access object when the owner is accessing it, it is safe for us to move the object and update the owner without need to concern about consistency and concurrency problem. The critical path in this whole process contains only one network trip.
% \mhr{One more complicated thing here is actually about Rust. Rust allows for owner read access when there are immutable references. But for simplicity, in the paper I just disable it, which does not affect correctness and expressiveness, but I am not sure if reviews are gonna ask about it if they are rust experts.}
% \yiying{don't think you can just ignore this. need to support it and discuss it in the paper.}
% Data access through owner can be mutable or immutable. During runtime, we can know the type of the access but we cannot know if there currently exists other references when the access type is immutable. So similar to immutable references, the owner also records two addresses. One for data address and one for data copy address. When doing dereferencing, it checks whether data address is local. If yes, just dereference it. If no, for immutable dereferencing, \tool follows the way we handle the immutable reference including checking hashmap, copy data to local, and inserting or updating entries. \tool also records the address of the cached copy to its copy field. And for mutable dereferencing, \tool needs to check if there exists local cache copies by checking its data copy field. If yes, it directly updates its data address field to point to the data copy address, deallocate the original copy on the remote server, and then delete the entry in the hashmap because the ownership model guarantees that there must be no references pointing to the same data now. And when the owner goes out of scope, it also needs to check its data copy field. If it is not empty, we need to deallocate both the original data and the cached copy in local memory. 
% Another thing that needs special handling is that when we transfer the ownership of a value from one server to another server, \tool needs to deallocate the cached copy on the source server if it exists.

\MyPara{Immutable Reference}
Data access in \tool via immutable references presents unique challenges and efficiencies. Unlike mutable references, which have exclusive rights to data, thus enabling straightforward data movement without concurrency or consistency concerns, immutable references allow multiple concurrent pointers to the same data. A key advantage here is the Rust ownership model, which ensures these references are read-only, significantly simplifying consistency maintenance.
In \tool, each immutable reference contains dual addresses: the original data location and the local data copy address. Accessing data through an immutable reference involves a two-tiered check in DRust: Firstly, the system verifies whether the original data is stored locally. If so, it facilitates direct data access. Conversely, if the data is located remotely and if there is no local data copy, as depicted in Figure~\ref{fig:immutable}, DRust initiates a systematic approach: (1) replicating the data object to a local memory address, denoted as $p$ (\textcircled{1}), and (2) updating the reference's local copy address to $p$ (\textcircled{2}), while maintaining the original remote data intact.

Furthermore, DRust employs a local hashmap on each server, functioning as a mechanism for tracking local copies. This hashmap, indexed by the original data addresses, encompasses entries that store the local copy address and a counter indicating the number of immutable references to the data on this server. Upon replicating remote data object to local memory, \tool inserts a corresponding entry into this hashmap(\textcircled{3}). This ensures that subsequent accesses to the same object can leverage local copies, akin to a cache hit. As shown in figure~\ref{fig:immutable}, \tool looks up the hashmap using the original data address as key, increments the reference count of the entry in the hashmap(\textcircled{4}) and updates the reference's local copy address field with the local address we get(\textcircled{5}).

The creation of new shared immutable references and the management of reference scope are also critical aspects. When generating new shared immutable references from existing ones, only the original data address is duplicated, leaving the new reference's local copy field null. This approach ensures the integrity of the reference count in the hashmap and ascertains that the local copy address is genuinely local. Subsequent data accesses through this new reference prompt \tool to update the local copy field and the hashmap accordingly.
In scenarios where an immutable reference becomes out-of-scope, DRust decrements the reference count in the hashmap(\textcircled{6}) before dropping the reference itself(\textcircled{7}), provided the local copy field is non-null. When this count drops to zero(\textcircled{9}), indicating the absence of alive references, DRust deallocates the local data copy(\textcircled{10}).
This system only incurs a single network trip for initial data access, effectively bypassing network synchronization overheads and primarily dealing with local synchronizations.



% While message passing is a more recommended way of handling concurrency in Rust, it also allows the use of another method to manage thread concurrency: Shared State, mainly including mutexes and atomic types. Mutex is an abbreviation for mutual exclusion, as in, a mutex allows only one thread to access some data at any given time. To access the data in a mutex, a thread must first signal that it wants access by asking to acquire the mutex’s lock. The lock is a data structure that is part of the mutex that keeps track of who currently has exclusive access to the data. Therefore, the mutex is described as guarding the data it holds via the locking system. Mutexes are mostly used together with Arc to let each thread be able to hold the ownership of it with immutable access right. Internally, it uses unsafe code to guarantee that at any time only one owner can mutate the value. (We will discuss how to handle custom unsafe code in \tool in section~\ref{sec:unsafe}.) \tool follows this rule and preserves our mechanism for Arc. We maintain only one copy of the mutex and its internal guarded data. The redesigned mutex is just a pointer pointing to the internal real mutex. The outer mutex can be freely copied to multiple machines through the Arc smart pointer. When the lock function of the mutex is called, we route the lock request to the server which stores the real mutex and data, and returns the data to the server requesting the access right. And after the data read/write finishes and the unlock method is called, we write back the data to its original location and tell the real mutex that other threads can compete for the value now. For atomic types, the mechanism is similar. Only one difference is we do not have lock/unlock methods for that. Instead, we just route every access request to the server which stores the real atomic value. 
% We can see that for shared states, since there is not much semantics for us to use to boost performance, 

% 

 % Rust allows a value to have multiple owners using the smart pointer Rc<T> or Arc<T> to create a reference counted value. They keep track of the number of references to a value to determine whether or not the value is still in use. If there are zero references to a value, the value can be cleaned up without any references becoming invalid. Since Rc<T> is only for use in single-threaded scenarios so it does not need changes even in our distributed setting. For Arc<T>, multiple owners in multiple threads on multiple server can coexist. But all of them can only have read access rights. So data access through reference counted smart pointer is almost the same as immutable references. The difference is just when the count value in the value entry decreases to 0, it does not deallocate the cache copy, but just keep it, so as to save future possible reread of the same data. This is because that we know this value can only be read at all time so it is safe to keep this cache copy in local memory. And when there is memory pressure on this machine (memory usage exceeds 90\%), we will drop the cached copies whose reference count is 0 using LRU policy.
% \yiying{What's your eviction policy here? you can't keep every cached copy forever, right?} 


% How to place data and compute is vital to application's performance in a distributed system. \tool prioritizes load balancing when scheduling compute by spawning threads to the server with most resources. However, this method does not consider locality information in the application. In this section, we introduce two novel language constructs in \tool. Programmers can use these constructs to easily express locality information including data-data locality and data-compute locality. \tool can use the information provided by programmers through these constructs to further optimize the application performance running on our DSM.


% Besides data-data locality, the locality relationship between compute and data is also very important. As shown in section~\ref{sec:std}, \tool's thread manager provides the same interface as Rust's original thread interface to save programmers' effort to learn new interface or modify their existing applications. Programmers can distribute the workload to other servers by spawning new threads. Then \tool just spawns the new thread to the server with most available resources to achieve load balancing. However this could cause inefficiencies. For example, what if data is located on one server but the thread executing the function that mostly accesses that data is scheduled to another server? Then clearly it is better if we can schedule that thread to the server containing the data it is going to access the most, so as to reduce data transfer between servers. To achieve this, the thread managers needs to gather semantics from programs about what data it is going to access the most. To get this information, we provide an interface to enable programmers express this semantics. Figure~\ref{lst:thread} shows an the example of this interface. This new interface accepts an additional argument of type Box<T>. It means the new thread it is going to spawn accesses this data structure the most. In that example, data of type D is created on a possibly remote server, then it uses the new interface to spawn the thread executing the compute\_func to the server containing the data pointed by d. Note that it is not guaranteed to schedule the thread at that server. The thread manager still checks whether the server holding the object pointed by this heap pointer has enough compute resource, if yes, it schedules the thread there. Otherwise, it follows traditional policy to spawn the new thread.




% This scheduling policy works well in our evaluation on three common workloads in data centers. \yiying{did you eval use different inputs?}


==> type.tex <==
\section{Formal Type System\label{sec:formal}}
% This section presents the formal semantics of core-\tool, a minimal formal language that consists of all important features of \tool. Core-\tool omits regular reference type because regular-typed references have the same property as local-typed references with only one difference: the object it points to is subject to swapping. It only affects performance but its usage is still like local-typed reference, so it does not affect our type system. 
This section provides the formal semantics for Core-\tool, a simplified formal language that encompasses the crucial features of \tool. It omits regular-typed data, as they behave similarly to local-typed data with only a slight performance difference due to the possibility of object swapping. Despite this, regular-typed data are still used in the same manner as local-typed data and do not impact our type system.

% We do not have functions in our type system. But we do have local and remote blocks which are executed on local/remote machines. Local/Remote blocks cannot read or write remote/local memory but they can transfer values between blocks.
Our type system does not include functions, but it does comprise local and remote blocks that run on local/remote machines. Local/Remote blocks are unable to access remote/local memory, but they can transfer values between each other.

\subsection{Syntax\label{sec:syntax}}



\[\begin{array}{rcrr} 
p & ::= & & \textrm{Places}\\
& & local & \textrm{in local}\\ 
&  & remote & \textrm{in remote}\\
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
t & ::=  & & \textrm{Terms}\\
&  & \{\overline{t}\}^l_p & \textrm{block}\\ 
&  & \textrm{let } p \textrm{ mut }x = t & \textrm{declaration}\\
& & w = t & \textrm{assignment}\\
& & p \textrm{ box } t & \textrm{heap allocation} \\
& & \&[\textrm{mut}]\textrm{ } w  & \qquad\textrm{(mutable) borrow}\\
& & w & \textrm{move}\\
& & \widehat{w} & \textrm{copy}\\
& & v & \textrm{value}\\
& & t \oplus t & \textrm{arithmetic} \\
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
w & ::= & & \textrm{LVals}\\
& & x & \textrm{variable}\\ 
&  & *w & \textrm{dereference}\\
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
v^{\bot} & ::= & & \textrm{Partial Values}\\
&  & v & \textrm{value}\\ 
&  & \bot& \textrm{undefined}\\ 
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
v^p& ::= & (v)_p  & \textrm{Placed Values}\\
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
v & ::= & & \textrm{Values}\\
& & \epsilon & \textrm{unit}\\
&  & c & \textrm{integer}\\
&  & l^{\bullet}, l^{\circ} & \textrm{reference}\\
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
\widetilde{T} & ::= & & \textrm{Partial Types}\\
& & T & \textrm{type}\\ 
&  &  (\Box \widetilde{T})_Q & \textrm{partial box}\\ 
&  & \lfloor T\rfloor& \textrm{undefined}\\ 
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
Q & ::= & & \textrm{Place Qualifiers}\\ 
&  & local & \textrm{local qualifier}\\ 
&  & remote & \textrm{remote qualifier}\\ 
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
B & ::= & & \textrm{Basic Types}\\ 
&  & \epsilon & \textrm{unit}\\ 
&  & \textrm{int} & \textrm{integer}\\ 
&  & \&[\textrm{mut}]\textrm{ } \overline{w} & \textrm{mutable borrow}\\ 
&  & \&\overline{w} & \textrm{immutable borrow}\\ 
&  &  \Box T & \textrm{box}\\ 
&  &  & \\
% \end{array}\]
% \[\begin{array}{rcrr} 
T & ::= & (B)_Q & \textrm{Types}\\ 
\end{array}\]

% \subsubsection{LVals}

% \[\begin{array}{lcr} 
% w & ::= & & \textrm{LVals}\\
% & ::= & x \\ 
% &  & *w
% \end{array}\]


% \subsubsection{Partial Values}

% \[\begin{array}{lcr} 
% % v^p& ::=& [ v^{\bot}]_p \\
% % & & \\
% v^{\bot} & ::= \\
% & & v \\ 
% &  & \bot
% \end{array}\]

% \subsubsection{Values}

% \[\begin{array}{lcr} 
% v^p& ::=& (v)_p \\
% & & \\
% v & ::= & \epsilon \\ 
% &  & c \\
% % &  & \dot{l}^{\bullet}, \dot{l}^{\circ} , \ddot{l}^{\bullet}, \ddot{l}^{\circ}
% &  & l^{\bullet}, l^{\circ}
% \end{array}\]

% \subsubsection{Partial Types}

% \[\begin{array}{lcr} 
% \widetilde{T} & ::= & T \\ 
% &  &  (\Box \widetilde{T})_Q \\
% &  & \lfloor T\rfloor
% \end{array}\]

% \subsubsection{Types}


% \[\begin{array}{lcr} 
% Q & ::= & local \\
% &  & remote \\
% & & \\
% B & ::= & \epsilon \\ 
% &  & \textrm{int} \\
% &  & \&[\textrm{mut}]\textrm{ } \overline{w} \\
% &  & \&\overline{w} \\
% &  &  \Box T \\
% & & \\
% T & ::= & (B)_Q
% \end{array}\]

\subsection{Operational Semantics}

\subsubsection{Helper Functions}


\paragraph{Local and Remote Memory} The partial function $Local(l)$ determines whether a given location is in local memory or not:

\[\begin{array}{rrll}
% local(l) & = & True & \textbf{if } l\mapsto \langle \cdot \rangle_{local}^m \in S  \\
local(l) & = & True & \textbf{if } l \textrm{ is in local memory}\\
% local(l)  & = & False & \textbf{if } l\mapsto \langle \cdot \rangle_{local}^m \notin S
local(l)  & = & False & \textbf{if }  l \textrm{ is in remote memory}
\end{array}\]

\paragraph{Locate} The partial function $loc_p(S, w)$ determines the location associated with a given lval in a given store and place.

\[\begin{array}{rrll}
loc_p(S,x) & = & l_x &\\
loc_p(S,*w) & = & l & \textbf{where } loc(S, w)=l_w \\
& & & \textbf{and } (S(l_w)={\langle \dot{l}^* \rangle}^m_p \textbf{ or } S(l_w)={\langle \ddot{l}^* \rangle}^m_p) \\

loc_p(S,w) & = & \bot & \textbf{otherwise}
\end{array}\]



\paragraph{Merge} We have 
$$\langle (\cdot)_p \rangle^m = \langle \cdot \rangle^m_p$$

% \paragraph{Read and Write} The partial function $read(S,w)$ retrieves the value stored in a given lval and the partial function write $write(S,w,v^\bot)$ updates the value stored in a given lval:

% \[\begin{array}{rrll}
% read(S,w) & = & S(l_w) & \textbf{where } loc(S,w)=l_w\\
% read(S,w) & = & \bot & \textbf{where } loc(S,w)=\bot\\
% write(S,w,v^\bot)  & = & S[l_w\mapsto \langle v^\bot\rangle^m] & \textbf{where } loc(S, w)=l_w \\
% & & & \textbf{and } S(l_w)=\langle \cdot \rangle^m\\
% write(S,w,v^\bot)  & = & S & \textbf{otherwise }
% \end{array}\]

\paragraph{Evaluation Context} An evaluation context is a term containing a single occurrence of $[\![\cdot]\!]$ (the hold) in place of a subterm. Evaluation context are defined as follows:
\[\begin{array}{rcl}
E & = & [\![\cdot]\!] \mid E;\overline{t} \mid \textrm{let } local \textrm{ mut }x = E \mid \textrm{let } remote \textrm{ mut }x = E \\
& & \mid w=E \mid local \textrm{ box } E \mid remote \textrm{ box } E \mid [\![\cdot]\!] \oplus E \\
& & \mid c \oplus E
\end{array}\]

\paragraph{Drop} Let $S$ be a program store. Then, the function $drop(S,m)$ is defined as $drop(S,\psi)$ where 
% $\psi=\{\dot{l}^\bullet | l\mapsto\langle v^\bot\rangle^m_{local}\in S\}\cup\{\ddot{l}^\bullet | l\mapsto\langle v^\bot\rangle^m_{remote}\in S\}$
$\psi=\{l^\bullet | l\mapsto\langle v^\bot\rangle^m_*\in S\}$
. Here, $drop(S,\psi)$ recursively deallocates owned locations as follows:

\[\begin{array}{rrll}
drop(S,\phi) & = & S \\
% drop(S,\psi \cup \{v^\bot\})  & = & drop(S, \psi) \\
% & & \textbf{if } v^\bot \neq \dot{l}^\bullet  \textbf{ and }  v^\bot \neq \ddot{l}^\bullet\\
drop(S,\psi \cup \{v^\bot\})  & = & drop(S, \psi) \quad \textbf{if } v^\bot \neq l^\bullet\\
drop(S,\psi \cup \{v^\bot\})  & = & drop(S-\{l\mapsto \langle v^\bot \rangle^*_* \}, \psi\cup\{v^\bot\}) \\
& & \textbf{where } S(l)=\langle v^\bot \rangle^*_*
\end{array}\]
 

\subsubsection{Expressions}


% \inferrule{R-Variable}{$S(l_x)=\langle b\rangle^m_p$}
% {$\langle$\step{$S \triangleright \widetriangle{x}$}{$S \triangleright [b]_p$}$\rangle^l_p$}

% \inferrule{R-Location}{$\langle$\step{$S \triangleright \widehat{w}$}{$S \triangleright [l_w]_p$}$\rangle^m_p$ $\quad S(l_w)=\langle b\rangle^m_p$}
% {$\langle$\step{$S \triangleright \widehat{*w}$}{$S \triangleright [b]_p$}$\rangle^l_p$}

%  -----------------------------------
 
% \inferrule{R-Copy}{$read(S,w)=\langle v \rangle^m_p$}
% {$\langle$\step{$S \triangleright \widehat{w}$}{$S \triangleright [v]_p$}$\rangle^l_p$}

\inferrule{R-Copy}{$loc_p(S,w) = l_w \quad S(l_w) = \langle v\rangle^m_p$}
{$\langle$\step{$S \triangleright \widehat{w}$}{$S \triangleright v$}$\rangle^l_p$}

% ---------------------------------------------

% \inferrule{R-Move}{$read(S,w)=\langle v \rangle^m_p\quad S_2=write(S_1,w,\bot)$}
% {$\langle$\step{$S_1 \triangleright w$}{$S_2 \triangleright [v]_p$}$\rangle^l_p$}

\inferrule{R-Move}{$loc_p(S_1,w) = l_w \quad S_1(l_w) = \langle v\rangle^m_p \quad S_2=S_1[l_w\mapsto \langle \bot\rangle^m_p]$}
{$\langle$\step{$S_1 \triangleright w$}{$S_2 \triangleright v$}$\rangle^l_p$}



% \inferrule{R-Box}{$l_n \notin dom(S_1)\quad p(l_n)\quad S_2 = S_1[l_n\mapsto  \langle b \rangle^m_p]$}
% {$\langle$\step{$S_1 \triangleright p \textrm{ box } b$}{$S_2 \triangleright [\dot{l}^\bullet_n]_p$}$\rangle^l_p$}

\inferrule{R-LocalBox}{$l_n \notin dom(S_1)\quad local(l_n)\quad S_2 = S_1[l_n\mapsto  \langle v \rangle^*_{local}]$}
{$\langle$\step{$S_1 \triangleright local \textrm{ box } v$}{$S_2 \triangleright %\dot{l}
l^\bullet_n$}$\rangle^l_{local}$}


\inferrule{R-RemoteBox}{$l_n \notin dom(S_1)\quad \neg local(l_n)\quad S_2 = S_1[l_n\mapsto  \langle v \rangle^*_{remote}]$}
{$\langle$\step{$S_1 \triangleright remote \textrm{ box } v$}{$S_2 \triangleright %\ddot{l}
l^\bullet_n$}$\rangle^l_{remote}$}

% -----------------------------------------------
% \inferrule{R-LocalBorrow}{$loc_p(S,w)=l_w \quad local(l_w)$}
% {$\langle$\step{$S \triangleright \&[\textrm{mut}]\textrm{ } w $}{$S \triangleright \dot{l}^\circ_w$}$\rangle^l_p$}


% \inferrule{R-RemoteBorrow}{$loc(S,w)=l_w \quad \neg local(l_w)$}
% {$\langle$\step{$S \triangleright \&[\textrm{mut}]\textrm{ } w $}{$S \triangleright \ddot{l}^\circ_w$}$\rangle^l_p$}

\inferrule{R-Borrow}{$loc_p(S,w)=l_w$}
{$\langle$\step{$S \triangleright \&[\textrm{mut}]\textrm{ } w $}{$S \triangleright l^\circ_w$}$\rangle^l_p$}

% ------------------------------------------------

\inferrule{R-Plus}{$c_1 \oplus c_2 = c$}
{$\langle$\step{$S \triangleright c_1 \oplus c_2 $}{$S \triangleright c$}$\rangle^l_p$}


\subsubsection{Statements}


% \inferrule{R-Assign}{
% \[\begin{array}{c}
% read(S_1,w)=\langle v^\bot_1 \rangle^m_p \quad S_2=drop(S_1, \{v^\bot_1\})\\
% S_3=write(S_2,w,v_2)
% \end{array}\]
% }
% {$\langle$\step{$S_1 \triangleright w = v_2$}{$S_3 \triangleright \epsilon$}$\rangle^l_p$}
\inferrule{R-Assign}{
\[\begin{array}{c}
loc_p(S_1, w) = l_w \quad S_1(l_w)=\langle v^\bot_1 \rangle^m_p \\
S_2=drop(S_1, \{v^\bot_1\}) \quad   loc_p(S_2, w)=l_w\\
S_2(l_w)=\langle \cdot \rangle^m_p \quad S_3=S_2[l_w\mapsto v_2]
\end{array}\]
}
{$\langle$\step{$S_1 \triangleright w = v_2$}{$S_3 \triangleright \epsilon$}$\rangle^l_p$}


\inferrule{R-LocalDeclare}{
$local(l_x) \quad S_2 = S_1[l_x\mapsto \langle v \rangle^l_{local}]$
}
{$\langle$\step{$S_1 \triangleright \textrm{let } local \textrm{ mut }x = v $}{$S_2 \triangleright \epsilon$}$\rangle^l_{local}$}

\inferrule{R-RemoteDeclare}{
$\neg local(l_x) \quad S_2 = S_1[l_x\mapsto \langle v \rangle^l_{remote}]$
}
{$\langle$\step{$S_1 \triangleright \textrm{let } remote \textrm{ mut }x = v $}{$S_2 \triangleright \epsilon$}$\rangle^l_{remote}$}

\inferrule{R-Seq}{
$S_2=drop(S_1, {v})$
}
{$\langle$\step{$S_1 \triangleright v;\overline{t}$}{$S_2 \triangleright \overline{t}$}$\rangle^l_p$}


\inferrule{R-BlockA}{
$\langle$\step{$S_1 \triangleright t_1$}{$S_2 \triangleright t_2$}$\rangle^m_{p'}$
}
{$\langle$\step{$S_1 \triangleright \{\overline{t_1}\}^m_{p'}$}{$S_2 \triangleright \{\overline{t_2}\}^m_{p'}$}$\rangle^l_p$}


\inferrule{R-BlockB}{
$S_2=drop(S_1, m)$
}
{$\langle$\step{$S_1 \triangleright \{v\}^m_{p^'}$}{$S_2 \triangleright v$}$\rangle^l_p$}


\inferrule{R-Sub}{
$\langle$\step{$S_1 \triangleright t_1$}{$S_2 \triangleright t_2$}$\rangle^l_p$
}
{$\langle$\step{$S_1 \triangleright E[\![t_1]\!]$}{$S_2 \triangleright E[\![t_2]\!]$}$\rangle^l_p$}

\subsection{Typing Rules}

We use flow-sensitive typing rules. Judgments have the form "$\Gamma_1\vdash {_{\sigma}\langle t:T\rangle^l_p} \dashv \Gamma_2$" which are taken to mean: First, within lifetime $l$ and block place $p$, term $t$ has type $T$ under typing environment $\Gamma_1$; and second, that evaluating term $t$ under typing environment $\Gamma_1$ produces the (potentially updated) environment $\Gamma_2$. As for the store typing $\sigma$, it is needed for locations "in flight".


\subsubsection{Preliminaries}

\paragraph{Copy Types} A type $T$ has copy semantics, denoted by $copy(T)$, when $T=(\textrm{int})_Q$ or $T=(\&\overline{w})_Q$.

\paragraph{Merge}

$$\langle(\cdot)_Q\rangle^m = \langle \cdot \rangle^m_Q$$

\paragraph{Outer Place}

\[\begin{array}{rcll}
place(\widetilde{T}) & = & Q & \textbf{if} \quad \widetilde{T}=(B)_Q \\
& & place(T) & \textbf{if} \quad \widetilde{T}=\lfloor T \rfloor ]
\end{array}\]

\paragraph{Type Strengthening} Let $\widetilde{T}_1$ and $\widetilde{T}_2$ be partial types. Then $\widetilde{T}_1$ strengthens $\widetilde{T}_2$, denoted as $\widetilde{T}_1 \sqsubseteq \widetilde{T}_2$, according to the following rules:

\inferrule{W-Reflex}{}
{$\widetilde{T}_1 \sqsubseteq \widetilde{T}_1$}

\inferrule{W-Box}{$\widetilde{T}_1 \sqsubseteq \widetilde{T}_2$}
{$(\Box \widetilde{T}_1)_Q \sqsubseteq (\Box \widetilde{T}_2)_Q$}

\inferrule{W-Borrow}{$\overline{u} \subseteq \overline{w}$}
{$(\&[\textrm{mut}]\textrm{ } \overline{u})_Q \sqsubseteq (\&[\textrm{mut}]\textrm{ } \overline{w})_Q$}

\inferrule{W-UndefA}{$T_1 \sqsubseteq T_2$}
{$\lfloor T_1 \rfloor \sqsubseteq \lfloor T_2 \rfloor$}

\inferrule{W-UndefB}{$T_1 \sqsubseteq T_2$}
{$T_1 \sqsubseteq \lfloor T_2 \rfloor$}

\inferrule{W-UndefC}{$ \widetilde{T}_1 \sqsubseteq \lfloor T_2\rfloor $}
{$(\Box \widetilde{T}_1)_Q \sqsubseteq \lfloor (\Box T_2)_Q \rfloor$}


\paragraph{Type Join} Let $\widetilde{T}_1$ and $\widetilde{T}_2$ be partial types. Then their join, denoted $\widetilde{T}_1 \sqcup \widetilde{T}_2$, is a partial function returning the strongest $\widetilde{T}_3$ such that  $\widetilde{T}_1\sqsubseteq\widetilde{T}_3$ nad $\widetilde{T}_2\sqsubseteq\widetilde{T}_3$

\paragraph{Environment Strengthening} Let $\Gamma_1$ and $\Gamma_2$ be typing environments. Then $\Gamma_1$ strengthens $\Gamma_2$ denoted $\Gamma_1\sqsubseteq \Gamma_2$, iff $dom(\Gamma_1)=dom(\Gamma_2)$ and for all $x\in dom(\Gamma_1)$ where $\Gamma_1(x)=\langle \widetilde{T}_1\rangle^l$, we $\Gamma_2(x)=\langle \widetilde{T}_2\rangle^l$ where $\widetilde{T}_1\sqsubseteq \widetilde{T}_2$

\paragraph{Environment Join} Let $\Gamma_1$ and $\Gamma_2$ be typing environments. Then their join, denoted $\Gamma_1 \sqcup \Gamma_2$, is a partial function returning the strongest $\Gamma_3$ such that  $\Gamma_1\sqsubseteq\Gamma_3$ nad $\Gamma_2\sqsubseteq\Gamma_3$

\paragraph{LVal Typing} An lval $w$ is said to be typed with respect to an environment $\Gamma$ and place $Q$, denoted ${^Q}\Gamma \vdash w:\langle \widetilde{T} \rangle^m$, according to the following rules:

% \paragraph{Write} Let $\Gamma$ be an environment where $\Gamma(x) = $

\inferrule{T-LvVar}{$ \Gamma(x) = \langle \widetilde{T} \rangle^m $}
{${^Q}\Gamma \vdash x:\langle \widetilde{T} \rangle^m$}

\inferrule{T-LvBox}{$ {^Q}\Gamma \vdash w:\langle \Box \widetilde{T} \rangle^m_Q $}
{${^Q}\Gamma \vdash *w:\langle \widetilde{T} \rangle^m$}

\inferrule{T-LvBor}{$ {^Q}\Gamma \vdash w: \langle \&[\textrm{mut}]\textrm{ }\overline{u} \rangle^n \qquad \overline{{^Q}\Gamma\vdash u_i:\langle B_i \rangle^{m_i}_Q} $}
{${^Q}\Gamma \vdash *w:\langle \sqcup_i (B_i)_Q \rangle^{\sqcap_i m_i}$}

\paragraph{Path} A path, $\pi$, is a sequence of zero or more path selectors, $\rho$, which is either empty ($\pi\triangleq \epsilon$) or composed by appending a selector onto another path ($\pi\triangleq \pi'\cdot \rho$).

\paragraph{Path Selector} A path selector, $\rho$, is always a dereference ($\rho \triangleq *$).

\paragraph{Path Conflict} Let $u\triangleq \pi_u\mid x$ and $w\triangleq \pi_w\mid y$ be lvals. Then $w$ is said to conflict with u, denoted $u\Join w$, if $x=y$.

\paragraph{Type Containment} Let $\Gamma$ be an environment where $\Gamma(x)=\langle\widetilde{T} \rangle^l$ for some $l$. Then $\Gamma\vdash x \leadsto T_y$ denotes that variable $x$ contains type $T_y$ and is defined as $contains(\Gamma,\widetilde{T},T_y)$ where:

\[\begin{array}{rrll}
contains(\Gamma, \widetilde{T}, T_y) & = & contains(\Gamma, \widetilde{T}', T_y) & \textbf{if } \widetilde{T} =(\Box\widetilde{T}')_*\\
& = & true & \textbf{if } \widetilde{T} =T_y\\
& = & false & \textbf{otherwise}
\end{array}\]

\mhr{The following rule borrowed from~\cite{pearce2021lightweight} is too strict. Acually as long as $w$ does not contain $u_i$, then it is fine to read. But we keep it as originial here for now.}
\paragraph{Read Prohibited} In an environment $\Gamma$, an lval $w$ is said to be read prohibited, denoted $readProhibited(\Gamma,w)$, when some $x$ exists where $\Gamma\vdash x\leadsto \&\textrm{mut }\overline{u}$ and $\exists_i(u_i\Join w)$

\paragraph{Write Prohibited} In an environment $\Gamma$, an lval $w$ is said to be write prohibited, denoted $writeProhibited(\Gamma,w)$, when some $x$ exists where $\Gamma\vdash x\leadsto \&\textrm{ }\overline{u} \wedge \exists_i(u_i\Join w)$, or $readProhibited(\Gamma, w)$ holds.

\paragraph{Move} Let $\Gamma$ be an environment where $\Gamma(x)=\langle\widetilde{T}_1\rangle^l$ for some lifetime $l$, and $w$ an lval where $w\triangleq \pi_x\mid x$. Then, $move(\Gamma, w)$ is a partial function defined as $\Gamma[x\mapsto\langle \widetilde{T}_2\rangle^l]$ where $\widetilde{T}_2=strike(\pi_x\mid \widetilde{T}_1)$:

\[\begin{array}{rrll}
strike(\epsilon\mid T) & = & \lfloor T\rfloor & \\
strike((\pi\cdot *)\mid (\Box \widetilde{T}_1)_Q) & = & (\Box \widetilde{T}_2)_Q & \textbf{where }\widetilde{T}_2=strike(\pi\mid\widetilde{T}_1)
\end{array}\]

\paragraph{Environment Drop} The environment drop deallocates locations by removing them from an environment, $\Gamma$, as follows: $drop(\Gamma, m)=\Gamma-\{x\mapsto  \langle \widetilde{T} \rangle^m \mid x\mapsto  \langle \widetilde{T} \rangle^m\in \Gamma\}$

\paragraph{Mutable} Let $\Gamma$ be an environment where $\Gamma(x)=\langle\widetilde{T}\rangle^l$ for some lifetime $l$, and $w$ an lval where $w\triangleq \pi_x\mid x$. Then $mut(\Gamma,w)$ is a partial function defined as $mutable(\Gamma, \pi_x\mid \widetilde{T})$ that determines whether $w$ is mutable:

\[\begin{array}{rrl}
mutable(\Gamma, \epsilon\mid T)& = & true \\
mutable(\Gamma, (\pi\cdot *)\mid\Box T)& = & mutable(\Gamma,\pi\mid T) \\
mutable(\Gamma, (\pi\cdot *)\mid\&\textrm{mut } \overline{w})& = & \wedge_i mut(\Gamma, \pi\cdot w_i)
\end{array}\]

\paragraph{Write} Let $\Gamma$ be an environment where $\Gamma(x)=\langle \widetilde{T}_1\rangle^l$ for some lifetime $l$ and lval $w$ where $w\triangleq\pi_x \mid x$. Then, $write^k(\Gamma,w,T)$ is a partial function defined as $\Gamma_2[x\mapsto \langle T_2\rangle^l]$ for some rank $k\geq 0$ where $(\Gamma_2,\widetilde{T}_2)=update^k(\Gamma, \pi_x\mid \widetilde{T}_1, T)$
\[\begin{array}{rrl}
update^0(\Gamma,\epsilon\mid\widetilde{T}_1, T_2)& = & (\Gamma,T_2) \\
update^{k\geq 1}(\Gamma,\epsilon\mid T_1, T_2)& = & (\Gamma,T_1\sqcup T_2) \\
update^{k}(\Gamma_1,(\pi\cdot *)\mid (\Box\widetilde{T}_1)_Q, T)& = & (\Gamma_2, (\Box \widetilde{T}_2)_Q) \\
\multicolumn{3}{r}{\textbf{where } (\Gamma_2, \widetilde{T_2}) = update^k(\Gamma_1,\pi\mid \widetilde{T}_1, T)} \\
update^{k}(\Gamma_1,(\pi\cdot *)\mid (\&\textrm{mut }\overline{u_i})_Q, T)& = & (\sqcup_i\Gamma_i, (\&\textrm{mut }\overline{u_i})_Q) \\
\multicolumn{3}{r}{\textbf{where } \Gamma_i=write^{k+1}(\Gamma,\pi\mid u_i,T)}\\
\end{array}\]

\subsubsection{Expressions}

% \inferrule{T-Const}{$\sigma\vdash v:T$}
% {$\Gamma\vdash {_\sigma}\langle v:T \rangle^l_Q\dashv \Gamma$}
\inferrule{T-Const}{$\sigma\vdash v:B \quad p=Q$}
{$\Gamma\vdash {_\sigma}\langle v:(B)_Q \rangle^l_p\dashv \Gamma$}


% \inferrule{T-Copy}{$\Gamma\vdash w:\langle B \rangle^m_Q\quad T=(B)_Q\quad copy(T) \quad \neg readProhibited(\Gamma,w)$}
% {$\Gamma\vdash {_\sigma}\langle \widehat{w}:B \rangle^l_Q\dashv \Gamma$}
\inferrule{T-Copy}{${^Q}\Gamma\vdash w:\langle B \rangle^m_Q\quad copy(T) \quad \neg readProhibited(\Gamma,w)\quad p=Q$}
{$\Gamma\vdash {_\sigma}\langle \widehat{w}:(B)_Q \rangle^l_p\dashv \Gamma$}

\inferrule{T-Move}{
\[\begin{array}{c}
{^Q}\Gamma_1\vdash w:\langle B\rangle^m_Q \quad \neg writeProhibited(\Gamma_1, w)  \\
\Gamma_2=move(\Gamma_1, w)\quad p=Q
\end{array}\]
}
{$\Gamma_1\vdash {_\sigma}\langle w:(B)_Q\rangle^l_p \dashv \Gamma_2$} 

\inferrule{T-MutBorrow}{${^Q}\Gamma\vdash w:\langle  B\rangle^m_Q\quad mut(\Gamma,w)\quad \neg writeProhibited(\Gamma,w)\quad p=Q$}
{$\Gamma \vdash {_\sigma}\langle \&\textrm{mut }w : \&\textrm{mut }w \rangle^l_p \dashv \Gamma$}

\inferrule{T-ImmBorrow}{${^Q}\Gamma\vdash w:\langle  B\rangle^m_Q\quad \neg readProhibited(\Gamma,w)\quad p =Q$}
{$\Gamma \vdash {_\sigma}\langle \&w : \&w \rangle^l_p \dashv \Gamma$}

% \mhr{The following one not right, needs reconsidering}
% \inferrule{T-Box}{$\Gamma_1 \vdash {_\sigma}\langle t :T \rangle^l_Q \dashv \Gamma_2$}
% {$\Gamma_1 \vdash {_\sigma}\langle \textrm{box }t : \Box T \rangle^l_Q \dashv \Gamma_2$}

\inferrule{T-Box}{$\Gamma_1 \vdash {_\sigma}\langle t :T \rangle^l_Q \dashv \Gamma_2 \quad p=Q$}
{$\Gamma_1 \vdash {_\sigma}\langle p \textrm{ box }t : (\Box T)_Q \rangle^l_p \dashv \Gamma_2$}

\subsubsection{Statements}

\inferrule{T-Seq}{$\Gamma_1\vdash {_\sigma}\langle t_1:T_1\rangle^l_p\dashv \Gamma_2 \quad \textrm{...} \quad \Gamma_n\vdash {_\sigma}\langle t_n:T_n\rangle^l_p\dashv \Gamma_{n+1}$}
{$\Gamma_1\vdash {_\sigma}\langle \overline{t}:T_n \rangle^l_p\dashv \Gamma_{n+1}$}

\inferrule{T-Block}{
\[\begin{array}{c}
\Gamma_1\vdash {_\sigma}\langle \overline{t}:(B)_{Q'} \rangle^l_{p'}\dashv \Gamma_2 \quad \Gamma_2\vdash (B)_{Q'}\succeq l \\
Q'=p'\quad Q=p\quad \Gamma_3=drop(\Gamma_2,m)]
\end{array}\]}
{$\Gamma_1\vdash {_\sigma}\langle \{\overline{t}\}^m_{p'}:(B)_Q \rangle^l_p\dashv \Gamma_3$}

% \inferrule{L-Int}{}
% {$\Gamma\vdash (\textrm{int})_Q\succeq (l,Q)$}

% \inferrule{L-Borrow}{$\overline{\Gamma\vdash u:\langle B\rangle^m_Q} \quad \overline{m\succeq l}$}
% {$\Gamma\vdash \&\textrm{[mut] }\overline{u}\succeq (l,Q)$}

% \inferrule{L-Box}{$\Gamma\vdash T\succeq (l,*)$}
% {$\Gamma\vdash (\Box T)_Q \succeq (l,Q)$}

\inferrule{L-Int}{}
{$\Gamma\vdash (\textrm{int})_Q\succeq l$}

\inferrule{L-Borrow}{$\overline{\Gamma\vdash u:\langle B\rangle^m_*} \quad \overline{m\succeq l}$}
{$\Gamma\vdash \&\textrm{[mut] }\overline{u}\succeq l$}

\inferrule{L-Box}{$\Gamma\vdash T\succeq l$}
{$\Gamma\vdash (\Box T)_Q \succeq l$}

\inferrule{T-Declare}{
\[\begin{array}{c}
p=Q\quad x\notin dom(\Gamma_1)\quad \Gamma_1\vdash{_\sigma}\langle t:(B)_Q\rangle^l_p\dashv \Gamma_2 \\
\Gamma_3=\Gamma_2[x\mapsto\langle B\rangle^l_Q]
\end{array}\]}
{$\Gamma_1\vdash {_\sigma}\langle \textrm{let }p \textrm{ mut }x=t:\epsilon \rangle^l_p \dashv \Gamma_3$}

\inferrule{T-Assign}{\[\begin{array}{c}
{^Q}\Gamma_1\vdash w:\langle \widetilde{T}_1\rangle^m \quad p=Q\quad \Gamma_1\vdash {_\sigma}\langle t:T_2\rangle^l_p \dashv \Gamma_2 \\
\Gamma_2\vdash \widetilde{T}_1\approx T_2 \quad \Gamma_2\vdash T_2\succeq m \\
\Gamma_3 = write^0(\Gamma_2,w,T_2) \quad \neg writeProhibited(\Gamma_3,w)
\end{array}\]}
{$\Gamma_1\vdash {_\sigma}\langle w=t:\epsilon\rangle^l_p \dashv \Gamma_3$}

\inferrule{S-Int}{}
{$\Gamma \vdash (int)_Q \approx (int)_Q$}

\inferrule{S-Box}{$\Gamma \vdash \widetilde{T}_1 \approx \widetilde{T}_2$}
{$\Gamma \vdash (\Box \widetilde{T}_1)_Q \approx (\Box \widetilde{T}_2)_Q$}

\inferrule{S-Borrow}{$\forall_{i,j}.(\Gamma\vdash u_i:\widetilde{T}_1\approx \widetilde{T}_2:w_j\dashv \Gamma) $}
{$\Gamma \vdash (\&\textrm{[mut] }\overline{u})_Q \approx  (\&\textrm{[mut] }\overline{w})_Q$}

\inferrule{S-UndefL}{$\Gamma \vdash T_1 \approx \widetilde{T}_2$}
{$\Gamma \vdash \lfloor T_1\rfloor \approx \widetilde{T}_2$}

\inferrule{S-UndefR}{$\Gamma \vdash \widetilde{T}_1 \approx T_2$}
{$\Gamma \vdash \widetilde{T}_1 \approx \lfloor T_2\rfloor $}


% \mhr{TODO: We need to prove that (1) well-typed program never got stuck, and can preserve well formedness; (2) Remote functions and local functions do not interfere with each other. There would not be any indeterministic state for every object.}


\subsection{Type Soundness\label{sec:soundness}}


\subsubsection{Valid States}

\paragraph{Valid Term} Let $t$ be a term where $\overline{v}\in t$ is the sequence of distinct values it contains. Then, $t$ is well-formed if $\neg \exists_{i,j}.(i\neq j \wedge \exists_{l^{\bullet}}.(v_i=v_j=l^{\bullet}))$.

\paragraph{Valid Store} Let $S$ be a program store where $\overline{v}\in t$ is the sequence of distinct values contained in any $l\in dom(S)$. Then, $S$ is said to be valid when $\neg \exists_{i,j}.(i \neq j \wedge \exists_{l^\bullet}.(v_i=v_j=l^\bullet))$.

\paragraph{Valid State} Let $S\triangleright t$ be a program state where both $S$ and $t$ are valid. Let $\overline{v}\in t$ and $\overline{u}\in t$ be the sequence of distinct values contained in (respectively) $S$ and $t$. Then, $S\triangleright t$ is valid when $\neg \exists_{i,j}.(i\neq j\wedge \exists_{l^\bullet}.(v_i=u_j=l^\bullet))$.

\subsubsection{Safe Abstractions}

\paragraph{Valid Type} Let $S$ be a program store, $(v^\bot)_p$ a partial value and $\widetilde{T}$ a partial type. Then, $(v^\bot)_p$ is abstracted by $\widetilde{T}$ in S, denoted $S\vdash (v^\bot)_p \thicksim \widetilde{T}$, according to the following rules:

\inferrule{V-Unit}{}
{$S\vdash \epsilon \thicksim \epsilon$}

\inferrule{V-Int}{$p=Q$}
{$S\vdash (c)_p \thicksim (int)_Q$}

\inferrule{V-Undef}{$p=Q$}
{$S\vdash (\bot)_p \thicksim \lfloor (B)_Q\rfloor$}

\inferrule{V-Borrow}{$p=Q\quad \exists_i.(loc_p(S,w_i)=l)$}
{$S\vdash (l^\circ)_p \thicksim (\&[\textrm{mut}] \overline{w})_Q$}

\inferrule{V-Box}{$p=Q\quad S(l^\bullet)=\langle v^\bot \rangle^l_{p'} \quad S\vdash (v^\bot)_{p'} \thicksim \widetilde{T} $}
{$S\vdash (l^\bullet)_p \thicksim (\Box \widetilde{T})_Q$}

\paragraph{Valid Store Typing} Let $S$ be a program store, $\sigma$ a store typing, and $t$ a term where $\overline{(v)_p}\in t$ is the sequence of distinct positioned values it contains. Then, $\sigma$ is valid for state $S\triangleright t$, denoted $S\triangleright t\vdash \sigma$, if $\forall i.(S\vdash (v_i)_{p_i}\thicksim (\sigma(v_i))_{Q_i})$ where $p_i=Q_i$.

\paragraph{Variable Projection} For a set of variable identifiers, $\phi$, $\Theta(\phi)=\{l_x\mid x\in \phi\}$.


% \mhr{Following needs modification.}
\paragraph{Safe Abstraction} Let $\Gamma$ be a typing environment and $S$ a program store. Let $\mathcal{L}$ represents the set of all heap locations $l_n$. Then, $S$ is safely abstracted by $\Gamma$, denoted $S\thicksim \Gamma$, iff $(dom(S)-\mathcal{L})=\Theta(dom(\Gamma))$ and for all $x\in dom(\Gamma)$, we have $(S\vdash (v^\bot)_p \thicksim \widetilde{T})$ where $S(l_x)=\langle v^\bot \rangle^l_p$ and $\Gamma(x)=\langle \widetilde{T} \rangle^l$

\paragraph{Well-formed Environment} A typing environment $\Gamma$ is well-fromed with respect to some lifetime $l$ iff: (i) for all $x\in dom(\Gamma)$ and $\overline{w}\in \textrm{LVal}$ where $\Gamma \vdash x \leadsto \&[\textrm{mut}]\overline{w}\wedge\Gamma(x)=\langle \cdot \rangle^n_p$, we have ${^*}\Gamma\vdash w:\langle T\rangle^n \wedge m \succeq n$; (ii) for all $x\in dom(\Gamma)$ where $\Gamma(x)=\langle \cdot \rangle^n$, we have $n\succeq l$.

\begin{theorem}[Borrow Invariance]
Let $S_1\triangleright t$ be a valid state; let $\sigma$ be a store typing where $S_1\triangleright t\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ and a place $p$ where $S_1\thicksim \Gamma_1$ and $\Gamma_2$ be an arbitrary typing environment; let $t$ be a term; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t:T\rangle^l_p\dashv \Gamma_2$, then $\Gamma_2[\gamma\mapsto \langle T\rangle^l]$ is well-formed with respect to $l$ for arbitrary $y\in fresh$.
\end{theorem}

\begin{theorem}[Progress]
Let $S_1\triangleright t_1$ be a valid state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$, then either $t_1 \in Value$ or $\langle S_1\triangleright t_1 \rightarrow S_2\triangleright t_2\rangle^l_p$ for some state $S_2 \triangleright t_2$.
\end{theorem}

% \paragraph{Proof} \mhr{TODO}

\begin{theorem}[Preservation] 
Let $S_1\triangleright t_1$ be a valid state and $S_2\triangleright v$ a terminal state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$ and $\langle S_1\triangleright t_1 \leadsto S_2\triangleright v\rangle^l_p$, then $S_2 \triangleright v$ remains valid where $S_2\thicksim \Gamma_2$ and $S_2\vdash v\thicksim T$.
\end{theorem}


\subsection{Determinism\label{sec:determinism}}

There would not be any indeterministic state for every object.
% We prove three properties of dRust's core type system. 

%\paragraph{Lemma 1} Any data can be referenced either locally or remotely.
% Haoran: Just repeating ownership. No need to prove that.

\mhr{Maybe need the following lemma when proving the theorem. Not sure if we really need that and how to formalize that.}
\begin{lemma}[Distinction] 
Local functions can only access local data. Remote functions can only access remote data.
\end{lemma}

\paragraph{Local Version Store} Let $S_1$ be an arbitrary valid store, we define its local version $S_2$ as follows: for all $l\in S_1$, if $S_1(l)=\langle v\rangle^m_{remote}$, then $S_2(l)=\langle v\rangle^m_{local}$; otherwise $S_2(l) = S_1(l)$.

% We define two terms $t_1$ and $t_2$ are similar to each other if $t_1$ and $t_2$ are the same except the place annotations of blocks. More formally, we have the following definition.
\paragraph{Local Version Term} Let $t_1$ be an arbitrary valid term, we define its lothickcal version $t_2$ as follows:
\[\begin{array}{rcl} 
t_2 = \{\overline{t}\}^l_{local} & \textbf{if} & t_1 = \{\overline{t}\}^l_{remote}  \\ 
t_2 = \textrm{let } local \textrm{ mut }x = t & \textbf{if} & t_1 = \textrm{let } remote \textrm{ mut }x = t \\
t_2 = local \textrm{ box } t & \textbf{if} & t_1 = remote \textrm{ box } t \\
t_2=t_1 & \multicolumn{2}{l}{\textbf{otherwise}}
\end{array}\]

\begin{theorem}[Determinism] 
Let $S_1\triangleright t_1$ be a valid state, and $S_2\triangleright t_2$ be its local version. let $\sigma_1$ be a store typing where $S_1\triangleright t_1\vdash \sigma_1$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_1'$ be a typing environment; and, let $T_1$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T_1 \rangle^l_p \dashv \Gamma_1'$ and $t_1 \in Value$, then $t_2=t_1$. If $\Gamma_1\vdash {_\sigma}\langle t_1:T_1 \rangle^l_p \dashv \Gamma_1'$ and $\langle S_1\triangleright t_1 \rightarrow S_1'\triangleright t_1'\rangle^l_p$ for some state $S_1' \triangleright t_1'$, then $\langle S_2\triangleright t_2 \rightarrow S_2'\triangleright t_2'\rangle^l_{local}$ where $S_2' \triangleright t_2'$ is the local version of $S_1' \triangleright t_1'$.
\end{theorem}
% \paragraph{Proof} \mhr{TODO}

==> type_proof.tex <==
% \newpage
% \section{Proof}

% % \mhr{TODO: Prove Borrow Invariance, progress, preservation and theorem in section~\ref{sec:soundness} and \ref{sec:determinism}.}
% \subsection{Preliminaries}

% \begin{lemma}[Safe Strengthening]
% Let $S$ be a program store; let $\Gamma$ be a well-formed typing environment where $S\thicksim\Gamma$; let $T_1$, $T_2$ be types where $T_1\sqsubseteq T_2$; and let $v$ be a value. If $S\vdash (v)_p\thicksim T_1$ then $S\vdash (v)_p\thicksim T_2$.
% \end{lemma}

% \begin{lemma}[Transitive Strengthening]
% Let $\widetilde{T}_1$, $\widetilde{T}_2$, $\widetilde{T}_3$ be partial types. If $\widetilde{T}_1 \sqsubseteq \widetilde{T}_2$ and $\widetilde{T}_2 \sqsubseteq \widetilde{T}_3$, then $\widetilde{T}_1 \sqsubseteq \widetilde{T}_3$.
% \end{lemma}

% \begin{lemma}[Location]
% \label{lemma:location}
% Let $S$ be a program store; let $\Gamma$ be a well-formed typing environment where $S\thicksim\Gamma$; let $\widetilde{T}$ be a partial type; let $m$ be a lifetime; and, let $w$ be an lval. If ${^Q}\Gamma\vdash w: \langle \widetilde{T}\rangle^m$, then $loc_p(S,w) = l_w$ for some location $l_w$ where $p=place(\widetilde{T})$ and $S(l_w) = \langle v^\bot \rangle^m_p$ and $S\vdash (v^\bot)_p \thicksim \widetilde{T}$ and $p=Q$.
% \end{lemma}

% \begin{lemma}[Drop Preservation]
% \label{lemma:droppreserve}
% Let $S$ be a program store; let $\Gamma$ be a well-formed typing environment with respect to a lifetime $l$ where $S\thicksim\Gamma$. Then, $drop(S,l)\thicksim drop(\Gamma,l)$.
% \end{lemma}

% \begin{lemma}[Update Preservation]
% \label{lemma:updatepreserve}
% Let $S$ be a program store; let $\Gamma$ be a well-formed typing environment; let $\widetilde{T}_1$, $\widetilde{T}_2$ be partial types; let $m$ be a lifetime; let $(v^\bot_1)_p$, $(v^\bot_2)_p$ be partial values where $S\vdash (v^\bot_1)_p\thicksim \widetilde{T}_1$ and $S\vdash v^\bot_2\thicksim \widetilde{T}_2$; let $m$ be a lifetime; and, let $w$ be an lval where $\Gamma\vdash w:\langle\widetilde{T}_1\rangle^m_Q$. If $S\thicksim \Gamma$, then $drop(S,\{v_2^\bot\})[l_w\mapsto (v_1^\bot)_p)]\thicksim write^0(\Gamma,w,\widetilde{T}_2)$ where $loc_p(S,w)=l_w$ and $S(l_w) = \langle \cdot \rangle^m_p$.
% \end{lemma}

% \begin{lemma}[Value Typing]
% \label{lemma:valuetyping}
% Let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$; let $\Gamma_2$ be a typing environment; let $\sigma$ be a store typing; let $T$ be a type; and, let $v$ be a value. If $\Gamma_1\vdash {_\sigma}\langle v:T\rangle^l_p\dashv \Gamma_2$, then $\Gamma_1=\Gamma_2$.
% \end{lemma}

% % \subsection{Borrow Invariance}
% % \begin{theorem}[Borrow Invariance]
% % Let $S_1\triangleright t$ be a valid state; let $\sigma$ be a store typing where $S_1\triangleright t\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ and a place $p$ where $S_1\thicksim \Gamma_1$ and $\Gamma_2$ be an arbitrary typing environment; let $t$ be a term; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t:T\rangle^l_p\dashv \Gamma_2$, then $\Gamma_2[\gamma\mapsto \langle T\rangle^l]$ is well-formed with respect to $l$ for arbitrary $y\in fresh$.
% % \end{theorem}
% % \begin{proof}
% % By structural induction on the structure of $t$ according to section~\ref{sec:syntax}:
% % \begin{itemize}
% %     \item Base Case $t\triangleq [v]$. By \texttt{T-Const}, $\Gamma_1=\Gamma_2$. If $v\neq [l^\circ]$, then follows trivially as add $\gamma\mapsto \langle T\rangle^l$ to $\Gamma_1$ cannot invalidate well-formedness (where $\sigma\vdash v:B$ and $T=(B)_Q$). Otherwise follows by definition of Valid Store Typing. \mhr{Do not understand why.}
% %     \item Base Case $t\triangleq [\widehat{w}]$. By \texttt{T-Copy} 
% % \end{itemize}
% % \end{proof}

% \subsection{Progress Lemma}
% \begin{theorem}[Progress]
% Let $S_1\triangleright t_1$ be a valid state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$, then either $t_1 \in Value$ or $\langle S_1\triangleright t_1 \rightarrow S_2\triangleright t_2\rangle^l_p$ for some state $S_2 \triangleright t_2$.
% \end{theorem}
% \begin{proof}
% By structural induction on the structure of $t$ according to section~\ref{sec:syntax}:
% \begin{itemize}
%     \item Base Case $t_1\triangleq [\widehat{w}]$. By \texttt{T-Copy}, $\Gamma_1\vdash w:\langle T \rangle^m$. By Lemma~\ref{lemma:location}, we have $loc_p(S,w)=l_w$ and $S(l_w) = \langle v\rangle^m_p$. Hence, \texttt{R-Copy} applies.
%     \item Base Case $t_1\triangleq [w]$. By \texttt{T-Move}, $\Gamma_1\vdash w:\langle T \rangle^m$. By Lemma~\ref{lemma:location}, \texttt{R-Move} applies.
%     \item Base Case $t_1\triangleq [\&[\textrm{mut}]\textrm{ }w]$. By either \texttt{T-ImmBorrow} or \texttt{T-MutBorrow}, $\Gamma_1\vdash w:\langle T\rangle^m$ and by Lemma~\ref{lemma:location} $loc_p(S_1,w)$ is defined. Hence, \texttt{R-Borrow} applies.
%     \item Base Case $t_1\triangleq [p \textrm{ box }v]$. Straightforward as \texttt{R-LocalBox} and \texttt{R-RemoteBox} applies for fresh location $l_n$.
%     \item Base Case $t_1\triangleq [\textrm{let }p\textrm{ mut }x=v]$. By \texttt{T-Declare} $x\notin dom(\Gamma_1)$. Then, since $S_1\thicksim \Gamma_1$, we have $(dom(S_1)-\mathcal{L})=\Theta(dom(\Gamma_1))$ by the definition of Safe Abstraction. By construction, $l_x\notint \mathcal{L}$ (i.e., it is not a heap location), hence, $l_x\notin dom(S_1)$ and \texttt{R-Declare} applies.
%     \item Base Case $t_1\triangleq [w=v]$. By \texttt{T-Assign} $\Gamma_1\vdash w:\langle \widetilde{T}\rangle^m$. By Lemma~\ref{lemma:location}, we have $loc_p(S_1,w)=l_w$ and $S_1(l_w)=\langle v^'\rangle^m_p$. Then, since $S_1\thicksim \Gamma_1$, we have $S=drop(S_1, \{v^'\})$ defined. So what we need to show now is that $loc_p(S,w)=l_w$ and $S(l_w)=\langle \cdot \rangle^m_p$. This will not hold only if $loc_p(S,w)$ traversed a location dropped between $S_1$ and $S$. By inspection of definition of Drop, such a location must be a heap location involved in a cycle with itself (e.g., $\{l_x\mapsto \langle\Box \Box \& x \rangle^l_p\}$ for $*x = v$). Since $S_1\thicksim \Gamma_1$, any cycle could only involve a borrow. Since $\neg writeProhibited(\Gamma_1, w)$ by \texttt{T-Assign}, \texttt{R-Assign} applies. 
%     \mhr{Need more explanation.}
%     \item Base case $t_1\triangleq [\{v\}^m_p]$. By inspection of definition of Drop, $drop(S_1, m)$ is defined. Hence, \texttt{R-BlockB} applies.
%     \item Inductive Cases $t_1\triangleq [\textrm{box }t_2]$ where $t_2\neq [v]$, $t_1\triangleq[\textrm{let mut }x=t_2]$ where $t_2\neq [v]$, $t_1 \triangleq [w=t_2]$ where $t_2\neq [v]$, $t\triangleq [\{\overline{t}\}^m_p]$ where $\overline{t}\neq [v]$. Follows by inductive hypothesis.
% \end{itemize}
% \end{proof}

% \subsection{Preservation Lemma}
% \begin{theorem}[Preservation] 
% Let $S_1\triangleright t_1$ be a valid state and $S_2\triangleright v$ a terminal state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$ and $\langle S_1\triangleright t_1 \leadsto S_2\triangleright v\rangle^l_p$, then $S_2 \triangleright v$ remains valid where $S_2\thicksim \Gamma_2$ and $S_2\vdash v\thicksim T$.
% \end{theorem}

% We divide the preservation theorem into three lemmas and prove them one by one.

% \begin{lemma}[Alias Preservation]
% Let $S_1\triangleright t_1$ be a valid state and $S_2\triangleright v$ a terminal state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$ and $\langle S_1\triangleright t_1 \rightarrow S_2\triangleright v\rangle^l_p$, then $S_2 \triangleright v$ remains valid.
% \end{lemma}
% \begin{proof}
% By case analysis on the structure of $t$ for terms that can reduce to a value in one step.
% \begin{itemize}
%     \item Base Case $t_1\triangleq [\widehat{w}]$. Straightforward. Observe $S_1=S_2$ by \texttt{R-Copy} and $\Gamma_1=\Gamma_2$ by \texttt{T-Copy}. Then, follows by \texttt{T-Copy} and $copy(T)$ implies $v\triangleq [l^\bullet]$ cannot hold.
%     \item Base Case $t_1\triangleq [w]$. By \texttt{R-Move}, $S_2=S_1[l_w\mapsto \langle \bot \rangle^m_p]$ for some $l_w\in dom(S_1)$. Since $S_1\triangleright \bot$ was valid, follows that $S_2$ is valid. Suppose $v\triangleq [l^\bullet]$ (since otherwise trivial). By inspection of definition of Write, follows that $v$ is not contained in $S_2$. Thus, validity of $S_2\triangleright v$ follows.
%     \item Base Case $t_1\triangleq [\&[\textrm{mut}]\textrm{ }w]$. Straightforward. Observe $S_1=S_2$ by \texttt{R-Borrow} and $\Gamma_1=\Gamma_2$ by both \texttt{T-ImmBorrow} and \texttt{T-MutBorrow}. Then, follows by \texttt{R-Borrow} as $v\triangleq [l^\circ]$.
%     \item Base Case $t_1\triangleq [p \textrm{ box }v_2]$. By both \texttt{R-LocalBox} and \texttt{R-RemoteBox}, $S_2=S[l_n\mapsto \langle v_2 \rangle^*_p]$ for some $l_n\notin dom(S_1)$. Since $S_1\triangleright v_2$ was valid, follows that $S_2$ is valid. Finally, follows by both  \texttt{R-LocalBox} and \texttt{R-RemoteBox} as $v=l^\bullet_n$.
%     \item Base Case $t_1\triangleq [\textrm{let }p\textrm{ mut }x=v_2]$. By \texttt{R-LocalDeclare} and \texttt{R-RemoteDeclare}, $S_2=S_1[l_x\mapsto \langle v \rangle^*_p]$ where $l_x\notin dom(S_1)$. Since $S_1\triangleright v_2$ was valid, follows that $S_2$ is valid. we have $(dom(S_1)-\mathcal{L})=\Theta(dom(\Gamma_1))$ by the definition of Safe Abstraction. Finally, follows by both \texttt{R-LocalDeclare} and \texttt{R-RemoteDeclare} as $v\triangleq[\epsilon]$.
%     \item Base Case $t_1\triangleq [w=v_2]$. By \texttt{R-Assign} $S=drop(S_1,\{v_1\})$ $S_2=S_1[l_w\mapsto \langle v_2 \rangle^m_p]$ where $loc_p(w)=l_w$ and $S_1(l_w)=\langle v_1\rangle^m_p$. Since $S_1\triangleright v_2$ was valid, follows that $S_2$ is valid. Finally, follows by both \texttt{R-Assign} as $v\triangleq[\epsilon]$.
%     \item Base case $t\triangleq [\{v\}^m_p]$. By \texttt{R-BlockB}, $S_2=drop(S_1, m)$. By \texttt{T-Block}, $\Gamma_2\vdash T \succeq l$ and, hence, validity of $S_1\triangleright t$ implies validity of $S_2\triangleright v$. \mhr{Why?}
% \end{itemize}
% \end{proof}


% \begin{lemma}[Value Preservation]
% Let $S_1\triangleright t_1$ be a valid state and $S_2\triangleright v$ a terminal state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$ and $\langle S_1\triangleright t_1 \rightarrow S_2\triangleright v\rangle^l_p$, then $S_2 \vdash v\thicksim T $.
% \end{lemma}
% \begin{proof}
% By case analysis on the structure of $t$ for terms that can reduce to a value in one step.
% \begin{itemize}
%     \item Base Case $t_1\triangleq [\widehat{w}]$. By \texttt{R-Copy}, we have $S_1(l_w)=\langle v\rangle^n_p$ where $loc_p(S_1,w)=l_w$. By $T-Copy$, ${^Q}\Gamma_1\vdash w:\langle T\rangle^m$ where $p=Q$. Hence, follows by Lemma~\ref{lemma:location}.
%     \item Base Case $t_1\triangleq [w]$. By \texttt{R-Move}, $S_1(l_w)=\langle v\rangle^n_p$ where $loc_p(S_1,w)=l_w$. By $T-Move$, ${^Q}\Gamma_1\vdash w:\langle T\rangle^m$ where $p=Q$. Hence, follows by Lemma~\ref{lemma:location}.
%     \item Base Case $t_1\triangleq [\&[\textrm{mut}]\textrm{ }w]$. Follows trivially by Lemma~\ref{lemma:location}. \mhr{Why?}
%     \item Base Case $t_1\triangleq [p \textrm{ box }v_2]$. By \texttt{T-Const}, $\sigma\vdash v_2:T_2$. By \texttt{R-LocalBox} and \texttt{R-RemoteBox}, $S_2=S_1[l_n\mapsto \langle  v_2\rangle^*_p]$ where $v=l_n^\bullet$. Hence, $S_2\vdash l_n^\bullet\thicksim \Box T_2$ follows trivially from Definition of Valid Type.
%     By both \texttt{R-LocalBox} and \texttt{R-RemoteBox}, $S_2=S_1[l_n\mapsto \langle v_2 \rangle^*_p]$ for some $l_n\notin dom(S_1)$. Since $S_1\triangleright v_2$ was valid, follows that $S_2$ is valid. Finally, follows by both  \texttt{R-LocalBox} and \texttt{R-RemoteBox} as $v=l^\bullet_n$.
%     \item Base Case $t_1\triangleq [\textrm{let }p\textrm{ mut }x=v_2]$. Straightforward, since $\Phi\vdash\epsilon \thicksim \epsilon$ by Definition of Valid Type.
%     \item Base Case $t_1\triangleq [w=v_2]$. Straightforward, since $\Phi\vdash\epsilon \thicksim \epsilon$ by Definition of Valid Type.
%     \item Base case $t\triangleq [\{v\}^m_p]$. Straightforward, since $\sigma\vdash v:T$ by \texttt{T-Const}.
% \end{itemize}
% \end{proof}

% \begin{lemma}[Store Preservation]
% Let $S_1\triangleright t_1$ be a valid state and $S_2\triangleright v$ a terminal state; let $\sigma$ be a store typing where $S_1\triangleright t_1\vdash \sigma$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_2$ be a typing environment; and, let $T$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T \rangle^l_p \dashv \Gamma_2$ and $\langle S_1\triangleright t_1 \rightarrow S_2\triangleright v\rangle^l_p$, then $S_2\thicksim \Gamma_2$.
% \end{lemma}
% \begin{proof}
% By case analysis on the structure of $t$ for terms that can reduce to a value in one step.
% \begin{itemize}
%     \item Base Case $t_1\triangleq [\widehat{w}]$. Follows immediately, as $S_1=S_2$ by \texttt{R-Copy} and $\Gamma_1=\Gamma_2$ by \texttt{T-Copy}.
%     \item Base Case $t_1\triangleq [w]$. By \texttt{R-Move}, $S_2=S_1[l_w\mapsto \langle \bot \rangle^m_p]$ for some $l_w\in dom(S_1)$. By \texttt{T-Move}, we have ${^Q}\Gamma_1\vdash w:\langle T_w\rangle^m$ and $\Gamma_2 = move(\Gamma_1, w)$ where $\neg writeProhibited(\Gamma_1, w)$. By the definition of Valid Type, $S\vdash (\bot)_p \thicksim \lfloor T_w\rfloor$ and, hence, $S_2\thicksim \Gamma_2$ follows, since $w$ is not borrowed.
%     \item Base Case $t_1\triangleq [\&[\textrm{mut}]\textrm{ }w]$. Follows immediately, as $S_1=S_2$ by \texttt{R-Borrow} and $\Gamma_1=\Gamma_2$ by both \texttt{T-ImmBorrow} and \texttt{T-MutBorrow}. 
%     \item Base Case $t_1\triangleq [p \textrm{ box }v_2]$. By both \texttt{R-LocalBox} and \texttt{R-RemoteBox}, $v_1=l^\bullet_n$ and $S_2=S_1[l_n\mapsto \langle v_2\rangle^*_p]$ for some $l_)n$ for some $l_n\notin dom(S_1)$. Hence $(dom(S_2)-\mathcal{L})=(dom(S_1)-\mathcal{L})$. By \texttt{T-Box}, $\Gamma_1\vdash {_\sigma}\langle v_2:T_2 \rangle^l_p \dashv \Gamma_2$ and $\Gamma_1=\Gamma_2$ follows by Lemma~\ref{lemma:valuetyping}. Thus, $S_2\thicksim \Gamma_2$ follows directly from $S_1\thicksim \Gamma_1$.
%     \item Base Case $t_1\triangleq [\textrm{let }p\textrm{ mut }x=v_2]$. By \texttt{R-LocalDeclare} and \texttt{R-RemoteDeclare}, $S_2=S_1[l_x\mapsto \langle v \rangle^l_p]$ where $l_x\notin dom(S_1)$. By \texttt{T-Declare} and Lemma~\ref{lemma:valuetyping}, $\Gamma_1\vdash \langle v_2:T_2 \rangle^l_p\dashv \Gamma_1$ follows. Hence, $\Gamma_2=\Gamma_1[x\mapsto \langle T_2\rangle^l]$ by \texttt{T-Declare}. Observe, $x\notin dom(\Gamma_1)$ implies $l_x\notin dom(S_1)$, hence, $(dom(S_2)-\mathcal{L})=dom(\Gamma_2)$. Thus, $S_2\thicksim \Gamma_2$ follows.
%     \item Base Case $t_1\triangleq [w=v_2]$. By \texttt{R-Assign} $S=drop(S_1,\{v_1\})$ $S_2=S[l_w\mapsto \langle v_2 \rangle^m_p]$ where $loc_p(w)=l_w$ and $S_1(l_w)=\langle v_1\rangle^m_p$. By \texttt{T-Assign}, ${^Q}\Gamma_1\vdash w:T_1$ where $S_1\vdash (v_1)_p\thicksim T_1$ by Lemma~\ref{lemma:location}. By \texttt{T-Assign} and Lemma~\ref{lemma:valuetyping}, $\Gamma_1\vdash {_\sigma}\langle v_2: T_2\rangle^l_p \dashv \Gamma_1$ follows and, hence, $\Gamma_2=write^0(\Gamma_1,w,T_2)$. Then, follows by Lemma~\ref{lemma:updatepreserve}, since $S_1\vdash (v_2)_p\thicksim T_2$.
    
%     Since $S_1\triangleright v_2$ was valid, follows that $S_2$ is valid. Finally, follows by both \texttt{R-Assign} as $v\triangleq[\epsilon]$.
%     \item Base case $t\triangleq [\{v\}^m_p]$. By \texttt{R-BlockB}, $S_2=drop(S_1, m)$. By \texttt{T-Block} and Lemma~\ref{lemma:valuetyping}, we have $\Gamma_1\vdash {_\sigma}\langle \rangle^m_p \dashv \Gamma_1$ follows. Hence, $\Gamma_2=drop(\Gamma_1,m)$. Then, $S_2\thicksim \Gamma_2$ by Lemma~\ref{lemma:droppreserve}.
% \end{itemize}
% \end{proof}



% \subsection{Determinism Theorem}
% \begin{theorem}[Determinism] 
% Let $S_1\triangleright t_1$ be a valid state, and $S_2\triangleright t_2$ be its local version. let $\sigma_1$ be a store typing where $S_1\triangleright t_1\vdash \sigma_1$; let $\Gamma_1$ be a well-formed typing environment with respect to a lifetime $l$ where $S_1\thicksim \Gamma_1$; let $\Gamma_1'$ be a typing environment; and, let $T_1$ be a type. If $\Gamma_1\vdash {_\sigma}\langle t_1:T_1 \rangle^l_p \dashv \Gamma_1'$ and $t_1 \in Value$, then $t_2=t_1$. If $\Gamma_1\vdash {_\sigma}\langle t_1:T_1 \rangle^l_p \dashv \Gamma_1'$ and $\langle S_1\triangleright t_1 \rightarrow S_1'\triangleright t_1'\rangle^l_p$ for some state $S_1' \triangleright t_1'$, then $\langle S_2\triangleright t_2 \rightarrow S_2'\triangleright t_2'\rangle^l_{local}$ where $S_2' \triangleright t_2'$ is the local version of $S_1' \triangleright t_1'$.
% \end{theorem}
% \begin{proof}
% \mhr{TODO}

% \end{proof}
